The Artin-Mazur zeta function for interval maps

In this work we study the Artin-Mazur zeta function for piecewise monotone functions acting on a compact interval of real numbers. In the case of unimodal maps, Milnor and Thurston gave a characterization for the rationality of the Artin-Mazur zeta function in terms of the orbit of the unique turning point. We show that for multimodal maps, the previous characterization does not hold.

==> Lorez-like_singularity.tex <==
\section{Proof of Proposition \ref{prop:0}}
In this section we will give the proof of Proposition \ref{prop:0}. We use the same notation as in the previous section. Let $h \colon [-1,1] \to [-1,1]$ be as in
Proposition \ref{prop:0} and $f = h \circ T \circ h^{-1}$. As in Theorem \ref{thm:1}, put 
$\tilde{c} \= h(0)$.

Since $h$ has a non-flat critical point at $0$, by \eqref{eq:right_crit_point} and \eqref{eq:left_crit_point} there are $\alpha^+ >0$, $\alpha^- >0$, and $\delta > 0$ such that
  \begin{equation}
    \label{eq:l_1}
    e^{-M}|\hat{x}|^{\alpha^+} \leq |h'(\hat{x})| \leq e^{M} |\hat{x}|^{\alpha^+},
  \end{equation}
  for every $\hat{x} \in (0,\delta)$ and

  \begin{equation}
    \label{eq:l_2}
    e^{-M}|\hat{x}|^{\alpha^-} \leq |h'(\hat{x})| \leq e^{M} |\hat{x}|^{\alpha^-},
  \end{equation}
  for every $\hat{x} \in (-\delta, 0)$.
% First, take $\delta > 0$ small enough so that $(-\delta,\delta) \subset I_k$ for some $k >2$.
% Since $h$ has a unique critical point at 
Since $c = 0$ and $c \notin I_k^1 = [c_{c_{S(k)+1}}, c_1],$ we have that there exist positive real numbers $W_1$ and $W_2$ such that for every
$x \in I_k$
\begin{equation}
  \label{eq:seq_bound}
  W_1 \leq |h'(T(x))| \leq W_2.
\end{equation}
\begin{proof}[Proof of Proposition \ref{prop:0}]
  
  By the chain rule we have
  \begin{equation}
    \label{eq:l_3}
    f'(x) = \lambda \frac{h'(T(h^{-1}(x)))}{h'(h^{-1}(x))},
  \end{equation}
  for every $x \in (h(-\delta), h(\delta)) \setminus \{ \tilde{c} \}.$ Let 
  $K \= \max \{ \lambda^{-1} e^M W_1^{-1}, \lambda e^M W_2 \}$. Then by \eqref{eq:seq_bound},
  \eqref{eq:l_1},
  \eqref{eq:l_2}, and \eqref{eq:l_3} we have that for every $x \in (\tilde{c}, h(\delta))$
  \begin{equation}
    \label{eq:l_6}
    \frac{1}{K|h^{-1}(x)|^{\alpha^+}} \leq |f'(x)| \leq \frac{K}{|h^{-1}(x)|^{\alpha^+}}, 
  \end{equation}
  and for every $x \in (h(-\delta), \tilde{c})$
  \begin{equation}
    \label{eq:l_7}
    \frac{1}{K|h^{-1}(x)|^{\alpha^-}} \leq |f'(x)| \leq \frac{K}{|h^{-1}(x)|^{\alpha^-}}.
  \end{equation}
 Now, from \eqref{eq:l_1} and \eqref{eq:l_2} there exist $M_1 >0$ and $M_2 > 0$ such that for every $x \in (0,\delta)
  $ \[ M_1^{-1} |x|^{\alpha^+ + 1} \leq |h(x)| \leq M_1 |x|^{\alpha^+ + 1}, \]
  and for every $x \in (-\delta,0)$
  \[ M_2^{-1} |x|^{\alpha^- + 1} \leq |h(x)| \leq M_2 |x|^{\alpha^- + 1}.  \]
  Since $h$ is a homeomorphism, there exist constants $M_3 > 0$ and $M_4 > 0$ such that  for every $x \in (\tilde{c}, h(\delta))$
  \begin{equation}
    \label{eq:l_4}
    M_3^{-1} |x - \tilde{c}|^{\frac{1}{\alpha^+ +1}} \leq |h^{-1}(x)| \leq 
    M_3 |x - \tilde{c}|^{\frac{1}{\alpha^+ + 1}}, 
  \end{equation}
  and for every $x \in (h(-\delta), \tilde{c})$
  \begin{equation}
    \label{eq:l_5}
    M_4^{-1} |x - \tilde{c}|^{\frac{1}{\alpha^- +1}} \leq |h^{-1}(x)| \leq 
    M_4 |x - \tilde{c}|^{\frac{1}{\alpha^- + 1}}.
  \end{equation}
  Then, by \eqref{eq:l_6}, \eqref{eq:l_7}, \eqref{eq:l_4}, and \eqref{eq:l_5}  we have that for every $x \in (\tilde{c}, h(\delta))$
  \[ \frac{1}{M_3 |x - \tilde{c}|^{\frac{\alpha^+}{\alpha^+ +1}}}  \leq 
  |f'(x)| \frac{M_3}{|x - \tilde{c}|^{\frac{\alpha^+}{\alpha^+ +1}}} , \]
  and for every $x \in (\tilde{c}, h(-\delta))$
  \[ \frac{1}{M_4 |x - \tilde{c}|^{\frac{\alpha^-}{\alpha^- +1}}} \leq 
  |f'(x)| \leq \frac{M_4}{|x - \tilde{c}|^{\frac{\alpha^-}{\alpha^- +1}}}. \]
  Thus, $f$ has a Lorenz-like singularity at $\tilde{c}$.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Unbounded_Lyapunov_exponent"
%%% End:


==> Proof_of_the_theorem.tex <==
\section{Proof of Theorem \ref{thm:1}}
In this section we will give the proof of Theorem 1. We will use the same notation as in the previous sections. 

First, note that if we put $\alpha \= \max \{ \alpha^+, \alpha ^- \} $, where $\alpha^+$ and $\alpha^-$ are given in Ptoposition \ref{prop:0}, from  \eqref{eq:thm_condition_1} and
\eqref{eq:thm_condition_2} we get that for every $x \in (h(-\delta), h(\delta)) \setminus \{ h(0) \}$
\begin{equation}
  \label{eq:thm_condition}
  \frac{1}{K |h'(h^{-1}(x))|^{\alpha}} \leq |f'(x)|.
\end{equation}
\begin{proof}
  Let us fix $k\geq 2$ big enough so that (\ref{eq:thm_condition}) holds on $I_k$ and such that $|f'\circ h| >1$ on $I_k$. For $n > k$ put $L_n \= \lambda^{S(n+1)}|D_n|.$ Define
  \[ \log|f'|^+ \= \max\{0,\log|f'|  \}\hspace{15pt} \text{ and } \hspace{15pt} \log|f'|^- \= \{0,-\log|f'|  \}. \]
  By Lemma \ref{lemm:J_k}, for every $n > k$, we have $J_n \subset I_k$ and for every 
  $k < n < n'$, we have $J_n \cap  J_{n'} = \emptyset$. So \[ \int \log|f'|^+d\tilde{\mu}_P \geq \int_{h(I_k)}\log|f'|d\tilde{\mu}_P\geq \sum_{n > k}\int_{h(J_n)}\log|f'|d\tilde{\mu}_P.\]
  Recall that $\varphi \= \frac{1 + \sqrt{5}}{2}$. Then  for each $n > k$ and $x \in J_n$, we have by (\ref{eq:thm_condition}) and(\ref{lemm:J_k})
  \begin{equation}
    \label{eq:f_derivative}
    |f'(h(x))| \geq  K^{-1} \frac{1}{|D_{n-1}|^{\alpha}} = K^{-1}\lambda^{\alpha S(n)} L_{n-1}^{-\alpha}. 
  \end{equation}
  %Let $M_n \= \log \left(\lambda K^{-1}\left[ \frac{1}{|D_0|} \prod_{i=0}^{n-2}C_i \right]^{\alpha}\right) $.
  By the above together with Lemma \ref{lemm:measure_estimate} and the fact that $S(n) \geq \frac{1}{3}\varphi^{n+2}$
  % \begin{eqnarray}
  %   \int_{h(J_n)} \log|f'|d\tilde{\mu}_P & \geq & \left( \frac{1}{\varphi} \right)^n \log{\left(\lambda K^{-1} \left( \frac{1}{|D_0|} \lambda^{S{(n)}} \prod_{i=0}^{n-2}C_i \right)^{\alpha}
  %                                                 \right)} \nonumber \\
  %                                        & = & \left( \frac{1}{\varphi} \right)^n \left[ \alpha S(n) \log(\lambda) + \log{\left(\lambda K^{-1}\left[ \frac{1}{|D_0|}
  %                                              \prod_{i=0}^{n-2}C_i \right]^{\alpha} \right)}  \right] \nonumber \\
  %                                        & = & \left( \frac{1}{\varphi} \right)^n \alpha \frac{1}{\sqrt{5}} \left( \varphi^n + \left( \frac{-1}{\varphi}  \right)^n  \right)
  %                                              \log(\lambda) + \left( \frac{1}{\varphi} \right)^n  M_n},  \nonumber \\
  %                                       & = & \frac{\alpha}{\sqrt{5}} \log(\lambda) + \alpha \left( \frac{-1}{\varphi^2} \right)^n\log{\lambda} + \left( \frac{1}{\varphi} \right)^n
  %                                              M_n, \nonumber
                                                %     \end{eqnarray}
  
  \begin{eqnarray}
    \int_{h(J_n)} \log|f'|d\tilde{\mu}_P & \geq & \tilde{\mu}_P(h(J_n)) \log \left| K^{-1} \lambda^{\alpha S(n)} L_{n-1}^{-\alpha}\right| \nonumber \\
                                         %& \geq & \left( \frac{1}{\varphi} \right)^n \log \left( \lambda K^{-1} \left( \frac{1}{|D_0|} \lambda^{S(n)} \prod_{i=0}^{n-2} C_i
                                                  %\right)^{\alpha}\right) \nonumber \\
                                         & \geq & \left( \frac{1}{\varphi} \right)^{n+1} \left[ \alpha S(n) \log(\lambda) + \alpha \log(K^{1/\alpha}L_n)^{-1}  \right] \nonumber \\
                                         & \geq & \frac{\varphi \alpha}{3}\log(\lambda) + \alpha \left( \frac{1}{\varphi} \right)^n \log(K^{1/\alpha}L_n)^{-1}.  \nonumber
  \end{eqnarray}
  By Lemma \ref{lemm:diam_estimate}, $\left( \frac{1}{\varphi} \right)^n \log(KL_n)^{-1} \longrightarrow 0$ as $n \longrightarrow 0$. We get that
  %Finally we get \[ \int \log|f'|^+d\tilde{\mu}_P \geq \sum_{n >k} \left[ \frac{\alpha}{3} \log(\lambda) + \alpha \left( \frac{1}{\varphi} \right)^n \log(KL_n)^{-1} \right].\]
                                                  %                                                   Since $\left( \frac{1}{\varphi} \right)^n M_n \to 0,$  we get that
  \begin{equation}
    \label{eq:positive_unbounded}
    \int \log|f'|^+d\tilde{\mu}_P = +\infty.  
  \end{equation}
  
  Now suppose by contradiction that 

  \begin{equation}
    \label{eq:finite_neg_int}
    \int \log|f'|^-d\tilde{\mu}_P < +\infty.
  \end{equation}
  By the chain rule
  
  \begin{equation}
    \label{eq:log_relation}
    \log|f'(x)| = \log(\lambda) + \log|h'(T(h^{-1}(x)))| - \log|h'(h^{-1}(x))|.
  \end{equation}
  Since $h'$ has a unique critical point, $\log|h'|$ is bounded away from the
  critical point, in particular is bounded from above in all $I$. Then $-\log|h'|$ is bounded from below on $I$. In particular, the integral
  \[ \int \log|h' \circ h^{-1}| d\tilde{\mu}_P,  \] is defined. Since the only critical points of $f$ are the points in
  $f^{-1}(\{c\})$, we have that $\log|f'|$ is bounded away from $\{\tilde{c}\} \cup f^{-1}\{\tilde{c} \}$. Let $\tV$ $\subset I \setminus \{c\}$ be a neighborhood of
  $f^{-1}\{ \tilde{c} \}$ such that $\log|f'(x)| < 0$ for $x \in \tV$, then by (\ref{eq:finite_neg_int}) and (\ref{eq:log_relation})
  \[ -\infty < \int_{\tilde{V}}\log|f'|d\tilde{\mu}_P = \log(\lambda)d\tilde{\mu}_P(\tilde{V}) + \int_{\tilde{V}}\left(\log|h'\circ T \circ h^{-1}| - \log|h' \circ h^{-1}|\right) 
    d\tilde{\mu}_P. \]  Since $h^{-1}(\tV)$ is a neighborhood of $T^{-1}(c)$, the function $-\log|h'\circ h^{-1}|$ is bounded on $\tV$. On the other hand, since
  \[T \circ h^{-1}(x) = c\] if  \[h^{-1} \circ f(x) = c,\] thus if \[f(x) = h(c) = \tilde{c}.\] So $h' \circ T \circ h^{-1}(x) = 0$ if $x \in f^{-1}(\tilde{c})$. Then
  $h' \circ T \circ h^{-1}(x) \neq 0$ for $x \in I \setminus \tV$. Then $\log|h' \circ T \circ h^{-1}|$ is bounded in $I \setminus \tV $, so
  \begin{equation}
    \label{eq:int_bound}
    \int_{I \setminus \tV}\log|h' \circ T\circ h^{-1}| d\tilde{\mu}_P > -\infty. 
  \end{equation}
  Now
  \begin{eqnarray}
    -\infty & < & \int_{\tilde{V}}\log|f'|d\tilde{\mu}_P \nonumber \\
            & \leq & \left( \log(\lambda)+ \max_{x \in \tilde{V}}\{-\log|h' \circ h^{-1}(x)|\}\right)\tilde{\mu}_P(\tilde{V}) + 
                     \int_{\tilde{V}}\left(\log|h'\circ T \circ h^{-1}| \right) d\tilde{\mu}_P. \nonumber 
  \end{eqnarray}
  So
  \begin{equation}
    \label{eq:other_inequality}
    \int_{\tilde{V}}\log|h' \circ T \circ h^{-1}| d\tilde{\mu}_P > - \infty.
  \end{equation}
  Together with (\ref{eq:int_bound}) this implies that \[\int\log|h' \circ T \circ h^{-1}| d\tilde{\mu}_P,\] is finite. Since the integral
  \[ \int -\log|h' \circ h^{-1}| d\tilde{\mu}_P, \] is defined, we have 
  
  \begin{eqnarray}
    \int \log|f'|d\tilde{\mu}_P & = & \log(\lambda) + \int \log|h'\circ T \circ h^{-1}|  d\tilde{\mu}_P  + \int- \log|h'\circ  h^{-1}| d\tilde{\mu}_P\nonumber \\
                                & = & \log(\lambda) + \int \log|h' \circ h^{-1} \circ f|  d\tilde{\mu}_P  + \int- \log|h'\circ  h^{-1}| d\tilde{\mu}_P.  \nonumber 
  \end{eqnarray}
  And since $\tilde{\mu}_P$ is $f$ invariant we get \[  \int \log|f'|d\tilde{\mu}_P  = \log(\lambda), \] contradicting (\ref{eq:positive_unbounded}). This contradiction completes
  the proof of the theorem.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Unbounded_Lyapunov_exponent"
%%% End:


==> Sec_4_Polynomial_dynamics.tex <==
\section{Dynamics of real polynomials} \label{section_polynomial_dynamics}

In this section, we present some general results on the dynamics of real 
polynomials.

Given $a, b \in \R$, we denote by $\langle a, b\rangle$ the convex hull of 
$\{ a,b \}$. Thus, in the case where $a \neq b$, the set
$\langle a, b\rangle$ is the smallest closed interval whose
boundary is equal to the set $\{ a,b\}$.

Let $f \colon \R \longrightarrow \R$ be a real polynomial of degree 
$d \geq 2$. We denote by $ \Crit (f) $ the set of critical points of $f$,
thus \[ \Crit (f) \= \{ x \in \R \colon f'(x) = 0 \}. \]

The \emph{real filled Julia set} of $f$, denoted by $K_{\R}(f)$, is the set
of all real numbers $x$ for which $\cO_f(x)$ is bounded (compare with the definition given in De Melo van Strien). This set coincides 
with the real trace of the filled Julia set of $f$ as a polynomial
acting on $\C$. Note that $K_{\R}(f)$ is compact, 

\begin{equation}
    \label{eq:invariance_of_filled_Julia}
   f(K_{\R}(f)) \subseteq K_{R} \hspace{1cm} \text{and} \hspace{1cm}
f^{-1}(K_{\R}(f)) \subseteq K_{\R}(f). 
\end{equation}


Observe that the set of periodic points of $f$ is contained in $K_{\R}(f)$,
then \[ \zeta_{f}(t) = \zeta_{f|_{K_{\R}(f)}}(t). \]

Given a periodic point $p$ of $f$ (or the cycle $\cO_{f} (p)$)  
its \emph{attracting basin} is defined as the set 
\[ \cB_f(p) \= \{x \in \R \colon p \in \omega_{f}(x) \}. \] 
Observe that if $p$ is attracting, then its basin contains an open set. 
The \emph{immediate attracting basin} of $p$, denoted by
$\widehat{\cB}_f(p)$, 
is the union of the connected components of its basin intersecting 
$\cO_{f}(p)$. If $\widehat{\cB}_f(p)$ is a neighbourhood of $\cO_f(p)$ then
this orbit is called a \emph{two-sided attractor}, otherwise we will say
that is a \emph{one-sided attractor}.


The \emph{basin of $f$}
is the union of the basins of its attracting periodic points, and we denote 
it by $\cB(f)$. The \emph{repeller} of $f$ is the set
\[ \Lambda (f) \= K_{\R}(f) \setminus \cB (f). \] 

% From now on, we will consider polynomial maps without critical points of 
% inflection type. So, every critical point is a local extremum. 

\begin{prop}
    Let $f \colon \R \longrightarrow \R$ be a polynomial map of degree 
    $d \geq 2$. If 
    $\Trn (f) \subset K_{\R}(f),$ then $K_{\R}(f)$ is connected and
    $f(\partial K_{\R}(f)) \subset \partial K_{\R}(f)$.
\end{prop}

\begin{proof}
    If $K_{\R}(f) = \emptyset$ the result is vacuously true. So, we assume 
    that $K_{\R}(f) \neq \emptyset$.

    If $\Trn (f) = \emptyset$, the map $f$ is monotone. Put 
    \[ c_0 \= \min (K_{\R}(f)) \hspace{0.5cm} \text{ and } \hspace{0.5cm}
    c_1 \= \max (K_{\R}(f)). \] Then $K_{\R}(f) \subset [c_0,c_1]$
    So, $K_{\R}(f) \subseteq [c_0, c_1]$. By monotonicity
    \begin{align*}
        f^n([c_0,c_1]) & \subseteq \langle f^n(c_0), f^n(c_1) \rangle \\
            & \subseteq [c_0,c_1].
    \end{align*}
    This implies that $[c_0,c_1] \subseteq K_{\R}(f)$.

    Suppose now that $\Trn (f) \neq \emptyset$, and put 
    \[ \Trn (f) \= \{ c_1, c_2, \ldots , c_n \}, \] with $1 \leq n \leq d-1$,
    \[ c_0 \= \min (K_{\R}(f)), \hspace{1cm} \text{and} \hspace{1cm} 
    c_1 \= \max (K_{\R}(f)).\] First, we prove that, in this case, 
    $\# K_{\R}(f) \geq 2$. If $K_{\R}(f)$ has a single element, this one 
    must be a fixed turning point. Thus \[ \Trn(f) = \{ c_1 \} =K_{\R}(f). \]
    Since $f$ is a polynomial, $c_1$ is a critical point of $f$. If $c_1$
    is a local minimum, $f|_{(c_1, \infty)}$ is increasing, and by the
    continuity of $f'$ and since $d \geq 2$, there exists $ \e >0$ so that $f(x) < x$ for every $x \in (c_1, c_1 + \e)$. On the other hand, for 
    every $x$ large enough, we have $f(x) > x$. Thus, there is an $x_0 > c_1$
    such that $f(x_0) = x_0$. In particular $x_0 \in K_{\R}(f)$, contradicting
    our assumption. So we must have \[ c_0 < c_{n+1}. \]
    
    Now, we will prove that $K_{\R}(f)$ is connected, thus we will prove
    that \[ K_{\R}(f) = [c_0, c_{n+1}] \]
    Since $\Trn (f) \subset K_{\R}(f)$, we have that 
    \[ f(\Trn (f))) \subset K_{\R}(f) \subset [c_0,c_{n+1}]. \] By 
    monotonicity, for every $0 \leq i \leq n$ we have  
    \[ f([c_i,c_{i+1}]) = \langle f(c_i), f(c_{i+1}) \rangle \subset 
    [c_0,c_{n+1}]. \] Thus, $f([c_0,c_{n+1}]) \subset [c_0,c_{n+1}]$. In 
    particular, for every $x \in [c_0,c_{n+1}]$, we have that 
    \[ \cO_{f}(x) \subset [c_0,c_{n+1}]. \] Thus, 
    $[c_0,c_{n+1}] \subset K_{\R}(f) $. This proves that 
    \[K_{\R}(f) = [c_0,c_{n+1}].\]

    %%%%%%%%%%%% PROOF BY CONTRADICTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Suppose that there is an $(c_0,c_n) \setminus K_{\R}(f)$ is nonempty. If 
    % $x \in (c_0,c_n) \setminus K_{\R}(f)$, then 
    % there exists a $k \geq 1$ so that $f^k(x) \notin [c_0, c_{n+1}]$. Put
    % \[ k_0 \= \min \{ n \geq 1 \colon f^k(x) \notin [c_0,c_{n+1}] \}, \] and 
    % \[ x_0 \= f^{k_0 -1}(x). \] So 
    % $x_0 \in [c_0, c_{n+1}] \setminus K_{\R}(f) $. Since 
    % $\Crit(f) \subset K_{\R}(f)$, the map $f$ is strictly monotone around 
    % $x_0$, and by continuity, there exist $\e >0$, and $1 \leq i \leq n-1$ 
    % so that 
    % \[ (x_0 - \e, x_0 +\e) \subset (c_i, c_{i+1}) \]  and 
    % \[ f((x_0 - \e, x_0 +\e)) \cap [c_0, c_{n+1}] = \emptyset. \]
    % As $f(c_i), f(c_{i+1}) \in [c_0, c_{n+1}]$, the above implies that there
    % is a critical point of $f$ in $(c_i, c_{i+1})$ whose image does not belong
    % to $[c_0, c_{n+1}]$. This contradicts our assumptions, so we must have 
    % that $K_{\R}(f)$ is connected, in particular 
    % \[K_{\R}(f) = [c_0, c_{n+1}],\] and $\partial K_{\R}(f) =\{c_0,c_{n+1}\}$.
    
    Now, we will prove that 
    $f(\partial K_{\R}(f)) \subset \partial K_{\R}(f)$. We start by proving 
    that $c_0, c_{n+1}$ are not turning points of $f$. Suppose that
    $c_0 \in \Trn (f)$. By definition of $c_0$, we have that 
    \[ (-\infty, c_0) \cap K_{\R}(f) = \emptyset. \] Since $c_0 \in \Trn (f)$
    there exists $\e > 0$ such that 
    \[ f((c_0 - \e, c_0)) \subset f((c_0, c_{n+1})) \subseteq K_{\R}(f). \]
    This cannot happen because of \eqref{eq:invariance_of_filled_Julia}. So,
    $c_0$ cannot be a turning point of $f$. 

    In the same way, it can be proved that $c_{n+1}$ cannot be a turning
    point of $f$.

    Finally, if $c_1$ is a local maximum (resp. local minimum), then 
    $f|_{(-\infty , c_1)}$ is increasing and $f(x) \rightarrow -\infty$ as 
    $x \rightarrow -\infty$ (resp. is decreasing and $f(x) \rightarrow 
    \infty$ as $x \rightarrow -\infty$). Thus, there exists a $c_{-1}$ in 
    $(-\infty , c_1)$ so that $f(c_{-1}) = c_0$ (resp. $f(c_{-1}) = c_{n+1} )$
    and  \[ f(-\infty, c_{-1}) \cap K_{\R}(f) = \emptyset. \]
    By \eqref{eq:invariance_of_filled_Julia}, $c_{-1} \in K_{\R}(f)$. This
    implies that $c_{-1}$ is the minimum of $K_{\R}(f)$, so $c_{-1}=c_0$.
    Thus, \[ f(c_0) \in \{ c_0, c_{n+1}\}. \]

    In the same way, it can be proved that 
    \[ f(c_{n+1}) \in \{ c_0, c_{n+1}\}. \]
\end{proof}


\begin{lemm}[ \cite{MevS93} ]
    \label{lemma:maps_without_fixed_points}
    Let $a,b \in \R$ with $a<b$. Let $f$ be a continuous function from 
    $[a,b]$ onto itself, without fixed points in $(a,b)$. Then, 
    $\Fix (f) = \{ a,b \}$, and either:
    \begin{enumerate}
        \item for all $x \in (a,b)$, $f(x) > x$ and 
        $\lim_{n \to \infty}f^n(x) = b$, or;
        \item for all $x \in (a,b)$, $f(x) < x$ and  
        $\lim_{n \to \infty}f^n(x) = a$. 
    \end{enumerate}
\end{lemm}

\begin{proof}
    Consider the continuous map $g \colon [a,b] \longrightarrow \R$ defined
    as $g(x) = f(x) - x$. Suppose that $f(a) > a$. 
    Since $f$ is onto, there must be a $x_0 \in (a,b]$ with 
    $f(x_0) = a < x_0$. So \[g(x_0) = a-x_0 < 0 < f(a)-a = g(a).\] By the 
    Intermediate Value Theorem, there exists a $y \in (a,x_0)$ such that 
    $g(y) = 0$, thus $f(y) = y$. This contradicts that $f$ has no fixed
    points in $(a,b)$. So we must have $f(a) = a$.

    In the same way, we can prove that $f(b) = b$ and that for every 
    $x \in (a,b)$, we have $f(x) > x$ or $f(x) < x$.

    Finally, for every $x \in (a,b)$, the sequence $\{ f^n(x) \}_{n \geq 0}$
    is increasing (resp. decreasing) if $x < f(x)$ (resp. $f(x) < x$). Then,
    it converges to some $y \in [a,b]$. Moreover,
    \[ f(y) = f(\lim_{n \to \infty} f^n(x)) = 
    \lim_{n \to \infty} f^{n+1}(x) = y. \] So $y$ is a fixed 
    point of $f$, then $y \in \{ a,b \}$. Since  $\{ f^n(x) \}_{n \geq 0}$
    is increasing (resp. decreasing), we have that $f^n(x) < y$ 
    (resp. $f(x)> y$) for all $n \geq 0$, so $y$ has to be equal to $b$
    (resp. $a$).
\end{proof}

Lemma \ref{lemma:maps_without_fixed_points} tell us that whenever we have a 
homterval for a map $f$ that is mapped onto itself without fixed points in
its interior, then its boundary consists of an attracting and a repelling 
fix point, and the homterval is contained in the immediate basin of 
attractions of the attracting fixed point in the boundary.

% Let $E$ be a subset of $\CC$. A map 
% \[ h \colon \D \times E \longrightarrow \CC \] is called a 
% \emph{holomorphic motion of $E$ parametrized by $\D$ and base point at 
% $0$} if 
% \begin{enumerate}
%     \item $h(0,z) = z$ for all $z \in E$,
%     \item for every $c \in \D$, the map $z \mapsto h(c,z)$ is injective on 
%     $\CC$, and 
%     \item for every $z \in E$ the map $c \mapsto h(c,z)$ is holomorphic for 
%     $c \in \D$.
% \end{enumerate}

% % Holomorphic motions were introduced by Ma\~n\'e, Sad, and Sullivan in their
% % study of the structural stability problem for complex rational maps, 
% % \cite{Mane-Sad-Sullivab_Lambda_lemma}. 
% % They proved the first result in the
% % topic which is called the $\Lambda$-lemma and which says that
% % any holomorphic motion $h(c, z)$ of $E$ parametrized by $\D$ and with base
% % point $0$ can be extended uniquely to a holomorphic motion of the closure 
% % of $E$.

% {\color{red} GENERALIZE THE RESULTS FOR PARAMETERS IN A POLIDISK. THUS, THE 
% POLYNOMIAL BEING PARAMETRIZED BY THE COEFFICIENTS}

% For the generalization above, we need to set the following notation in this section. Recall that,
% for $d \geq 3$, $1 \leq \nu \leq d-1$, and 
% $\boldsymbol{\mu} = (\mu_1, \ldots, \mu_{\nu}) \in \Z_{+}^{\nu}$, with $\sum_{i=1}^{\nu}\mu_i = d-1$,
% we denote by $\cP_d^{\boldsymbol{\mu}}(\R)$ the set of real polynomials of degree $d$ and $\nu$ distinct
% critical points of multiplicity 

% \begin{prop}
%     \label{prop:conjugacy_with_Fib_SFT}
%     Let $f_s \colon \R \longrightarrow \R$ be a family of real polynomials
%     of degree $d \geq 2$, 
%     whose coefficients depend real analytically on 
%     $s \in (s_1,s_2) \subset \R$.
%     Suppose that there is an $s_0 \in (s_1,s_2)$ such that 
%     $\Crit (f_{s_0}) \subset \R$, and $f_{s_0}$ has a 
%     real critical point $c$ that is a local extremum and is periodic
%     of minimal period three. Let $I$ be the smallest closed interval containing
%     $\cO_{f_{s_0}}(c)$ (thus, $I$ is the convex hull of $\cO_{f_{s_0}}(c)$). 
%     If $\interior (I) \cap \Crit (f_{s_0}) = \{ c \}$ 
%     then $\Lambda (f_{s_0}) \cap I$ is a Cantor set
%     contained in the interior of $I$,
%     and the action of $f_{s_0}$ restricted to it is topologically 
%     conjugate to the action of the left shift map $\sigma$ on $\SFib$. 
%     Moreover, there is a holomorphic motion $h$ of $\Lambda (f_{s_0}) \cap I$
%     defined on a neighborhood $\Omega$ of $s_0$ in $\C$ such that for every 
%     $s \in \Omega \cap (s_1,s_2)$ we have that
%     \[ h(s, \Lambda(f_{s_0}) \cap I) = \Lambda (f_{s}) \cap I. \]
    
    
% \end{prop}

% \begin{proof}
%     Without loss of generality, we assume that the shape of $f_{s_0}|_I$ 
%     is $(+,-)$.
%     In this case, we have $ f_{s_0}^2(c) < c < f_{s_0}(c) $, and thus 
%     $I = [f_{s_0}^2(c), f_{s_0}(c)]$. Put $I_1 \= [f^2_{s_0}(c), c]$, and
%     $I_2 \= [c, f_{s_0}(c)]$, so $f_{s_0}(I_1) = I_2$, and 
%     $f_{s_0}(I_2) = I$. We will say that a point
%     $x \in I_i \setminus \cO_{f_{s_0}}(c)$ has a 
%     \emph{symmetric with respect to $c$}, or just that it has a symmetric,
%     if there is a $\hat{x} \in I \setminus I_i$ such that 
%     $f_{s_0}(\hat{x}) = f_{s_0}(x)$. Observe that every 
%     $x \in \interior (I_1)$ 
%     has a symmetric, but if $\tilde{c} \in I_2$ is so that 
%     $f_{s_0}(\tilde{c}) = c$, then no point in $[\tilde{c} , f_{s_0}(c))$ 
%     has a symmetric.
    
%     The immediate basin of attraction of 
%     $\cO_{f_{s_0}}(c)$ restricted to $I$ is the union of the three intervals
%     $[f_{s_0}^2(c), p_2)$, $(\hat{p}_0, p_0)$, and $(p_1, f_{s_0}(c)]$, 
%     where $p_0$ is a periodic point of period three with 
%     $f_{s_0}(p_0) = p_1$, and $f_{s_0}^2(p_0) = p_2$, and 
%     $\hat{p}_0$ is the symmetric of $p_0$. 

%     First, we will construct the inverse branches of $f_{s_0}$ and $f_{s_0}^2$
%     on a suitable subinterval of $I$ and will extend this construction
%     to $f_s$ with $s$ in a neighborhood of $s_0$ in $\C$.
    
%     Since $c$ is periodic of period three, 
%     $\Crit (f_{s_0}) \cap \interior(I) = \{c\}$, and 
%     $\partial I \subset \cO_{f_{s_0}}(c)$, we have that, $f^3_{s_0}$ is a 
%     bijection from the interval $[f^2_{s_0}(c), p_2]$ onto
%     itself, and $f^2_{s_0}(c)$ is an attracting fixed point of $f^3_{s_0}$.
%     Since $[f^2_{s_0}(c), p_2)$ is contained in $\widehat{\cB}_{f_{s_0}}(c)$
%     there are no fixed points of $f^3_{s_0}$ in its interior. So
%     by Lemma~\ref{lemma:maps_without_fixed_points}, for all 
%     $x \in (f^2_{s_0}(c), p_2) $, we have that $f^3_{s_0}(x) < x$.
    
%     Fix $\ell_0 \in (f_{s_0}^2(c),p_2)$. We have 
%     \[ f_{s_0}(\ell_0) \in (c, p_0), \hspace{0.6cm} 
%     f_{s_0}^2(\ell_0) \in (p_1,f_{s_0}(c)), \hspace{0.3cm}
%     \text{ and } \hspace{0.3cm} 
%     f_{s_0}^3(\ell_0) \in (f_{s_0}^2(c), \ell_0). \]
%     Let $\ell_1 \in (f_{s_0}^3(\ell_0), \ell_0)$. Then, 
%     \[f_{s_0}(\ell_1) \in (c, f_{s_0}(\ell_0)), \hspace{0.5cm}  \text{ and }
%     \hspace{0.5cm}
%     f_{s_0}^2(\ell_1) \in (f_{s_0}^2(\ell_0), f_{s_0}(c)).\]

%     Let $\widehat{f_{s_0}(\ell_0)}$ be the symmetric of $f_{s_0}(\ell_0)$,
%     and put 
%     \[ J \= (f_{s_0}^3(\ell_0), f_{s_0}^2(\ell_1)),  \hspace{0.5cm}
%     J_1 \= (\ell_1, \widehat{f_{s_0}(\ell_0)}), \hspace{0.5cm} \text{ and } 
%     \hspace{0.5cm} J_2 \= (f_{s_0}(\ell_1), f_{s_0}^2(\ell_0)).\] Then, 
%     $\overline{J_i} \subset J$, $c \notin \overline{J_i}$ for $i = 1,2$, 
%     $\overline{J_1} \cap \overline{J_2} = \emptyset$, $f_{s_0}(J_1) = J_2$, 
%     and $f_{s_0}(J_2) = J$, see Figure \ref{fig:intervals_Js}.

%     Since \[\overline{J_i} \cap (\Crit (f_{s_0}) \cup f_{s_0}(\Crit (f_{s_0})) 
%     = \emptyset,\] 
%     the restrictions 
%     \[ f_{s_0}|_{J_2} \colon J_2 \longrightarrow J \hspace{0.5cm} 
%     \text{ and } \hspace{0.5cm} f^2_{s_0}|_{J_1} \colon J_1 \longrightarrow
%     J,\]
%     are diffeomorphisms. So, the inverse branches of $f_{s_0}$ and $f_{s_0}^2$
%     restricted to $J$, are well defined. Put 
%     \[ \phi_{s_0,2} \colon J \longrightarrow J_2 \hspace{0.5cm} 
%     \text{ and } \hspace{0.5cm} \phi_{s_0,1} \colon J \longrightarrow
%     J_1,\] with $\phi_{s_0,1} \= (f^2_{s_0}|_{J_1})^{-1}$,
%     and $\phi_{s_0,2} \= (f_{s_0}|_{J_2})^{-1}$. Also, since the critical 
%     points of $f_{s_0}$ are all real, the inverse branches, $\phi_{s_0,2}$ and $\phi_{s_0,1}$ extend uniquely to $\C_{J}$. So 
%     \[ \phi_{s_0,1} \colon \C_{J} \longrightarrow \C_{J_1} \hspace{0.5cm} 
%     \text{ and } \hspace{0.5cm} \phi_{s_0,2} \colon \C_{J} 
%     \longrightarrow \C_{J_2},\] are holomorphic. 

%     Fix $\theta \in (0, \pi)$. 
%     By the definition of $J_1$ and $J_2$, we have that 
%     \[ \phi_{s_0,1}(J) = J_1 \subset J \hspace{0.5cm}
%     \text{ and } \hspace{0.5cm} 
%     \phi_{s_0,2}(J) = J_2 \subset J.\] Then, by
%     Lemma \ref{lemm:Schwarz_Lemma}, we have that 
%     \begin{equation}
%         \label{eq:Schwarz_Lemma_hypothesis_for_phi_{s_0,i}}
%         \phi_{s_0,i}(D_{\theta}(J)) \subset D_{\theta}(J_i) \subset 
%         D_{\theta}(J). 
%     \end{equation}
%     Moreover, since $\overline{J_i} \subset J$, we have
%     \[ \overline{D_{\theta}(J_i)} \subset D_{\theta}(J). \] So   
%     \begin{equation}
%     \label{eq:Schwarz-Pick_hypohtesis_for_phi_{s_0,i}}
%     \overline{\phi_{s_0,i}(D_{\theta}(J))} \subset \overline{D_{\theta}(J_i)}
%     \subset D_{\theta}(J).
%     \end{equation}
%     Consider open intervals $K_1$ and $K_2$ satisfying the following:
%     \begin{enumerate}
%         \item $\overline{K_i} \subset J$, for $i = 1,2$;
%         \item $\overline{J_i} \subset K_i$, for $i =1,2$;
%         \item $\overline{K_1} \cap \overline{K_2} = \emptyset$;
%         \item $ c \notin \overline{K_1} \cup \overline{K_2}$.
%     \end{enumerate}
%     In particular, for $i = 1,2$
%     \[\overline{D_{\theta}(J_i)} \subset D_{\theta}(K_i) \hspace{0.5cm}
%     \text{ and } 
%     \hspace{0.5cm} \overline{D_{\theta}(K_i)} \subset D_{\theta}(J).\]
%     So, by \eqref{eq:Schwarz-Pick_hypohtesis_for_phi_{s_0,i}}
%     \begin{equation}
%         \label{eq:Image_of_D_theta_K_i}
%         \overline{D_{\theta}(J)} \subset f^2_{s_0}(D_{\theta}(K_1)) 
%         \hspace{0.5cm} \text{ and } \hspace{0.5cm}
%         \overline{D_{\theta}(J)} \subset f_{s_0}(D_{\theta}(K_2)).
%     \end{equation}    
%     Since the coefficients of $f_s$ depend real analytically on 
%     $s \in [a,b]$, there exists a neighborhood $\Omega \subset \C$ 
%     containing $s_0$ such that the coefficients extend to complex analytic
%     functions in $\Omega$. 
    
%     Using that  
%     \[ (\Crit (f_{s_0}) \cup f_{s_0}(\Crit (f_{s_0})) \cap 
%     \left(\overline{D_{\theta}(K_1)} \cup \overline{D_{\theta}(K_2)} \right) 
%     = \emptyset,  \] \eqref{eq:Image_of_D_theta_K_i}, and the Open Mapping 
%     Theorem, we can choose $\Omega$ to be small enough so that 
%     for every $s \in \Omega$ we have
%     \begin{equation}
%         \label{eq:f_s_containsD(J)}
%       \overline{D_{\theta}(J)} \subset f^2_{s}(D_{\theta}(K_1)) 
%     \hspace{0.5cm} \text{ and } \hspace{0.5cm}
%     \overline{D_{\theta}(J)} \subset f_{s}(D_{\theta}(K_2)),  
%     \end{equation}
%     and
%     \begin{equation}
%         \label{eq:no_crit_in_D(K_i)}
%         (\Crit (f_{s}) \cup f_{s}(\Crit (f_{s})) \cap 
%     \left(\overline{D_{\theta}(K_1)} \cup \overline{D_{\theta}(K_2)} \right) 
%     = \emptyset.
%     \end{equation}
%     Additionally, if $s \in \Omega \cap \R$, then $I \setminus \ov{K_1} \cup 
%     \ov{K_2}$ intersects a unique attracting cycle of period three and 
%     $\ov{K_1}$ and $\ov{K_2}$ intersect each component of the immediate basin
%     of this attracting cycle. These two conditions are to ensure that, 
%     for all $s \in \Omega \cap \R$, we have 
%     $\Lambda (f_s) \cap I \subset K_1 \cup K_2$, thus 
%     \[ \Lambda (f_s) \cap I = \{ x \in I \colon f_s^n(x) \in K_1 \cup K_2 
%     \text{ for all } n \geq 0 \}.\]
    
    
%     Conditions \eqref{eq:f_s_containsD(J)} and \eqref{eq:no_crit_in_D(K_i)}
%     allow us to define the inverse branches of $f_s$ and 
%     $f_s^2$ restricted to $D_{\theta}(K_1)$ and $D_{\theta}(K_2)$ 
%     respectively, for every $s \in \Omega$.
    
%     Put 
%     \[ \phi_{s,1} \= (f_s^2|_{D_{\theta}(K_1)})^{-1} \colon D_{\theta}(J)
%     \longrightarrow D_{\theta}(K_1) \]  and 
%     \[ \phi_{s,2} \= (f_s|_{D_{\theta}(K_2)})^{-1} \colon D_{\theta}(J)
%     \longrightarrow D_{\theta}(K_2).\]
%     Now, for $i = 1,2$, and every $s \in \Omega$, we have 
%     \begin{equation}
%     \label{eq:Unif_Cauchy_hyp}
%     \overline{\phi_{s,i}(D_{\theta}(J))} \subset \overline{D_{\theta}(K_i)}
%     \subset D_{\theta}(J).
%     \end{equation}
%     Thus, the image of $D_{\theta}(J)$
%     under $\phi_{s,i}$ is compactly contained in $D_{\theta}(J)$. Then, 
%     for every $s \in \Omega$, the maps $\phi_{s,1}$ and $\phi_{s,2}$ 
%     satisfies the hypothesis of Lemma \ref{lemm:uniform_contraction}. So, 
%     for every $\bf{w} = (w_i)_{i \geq 0} \in \{ 1,2 \}^{\N_0}$ and 
%     $k \geq 0$, if we put 
%     \[\phi_{s,\bf{w}|_{[0,k]}} \= \phi_{s,w_0} \circ \phi_{s,w_1} \circ \ldots
%     \circ \phi_{s,w_k},\] then 
%     $\{ \phi_{s,\bf{w}|_{[0,k]}} \}_{k \geq 0}$ converges
%     uniformly on $D_{\theta}(J)$ to a constant function. We write 
%     $\phi_{s,\bf{w}}$ for its limit, and $x_s(\bf{w})$ for the value of 
%     $\phi_{s,\bf{w}}$ in $D_{\theta}(J)$.
%     %%%%%%reviewed until here continue tomorrow    

%     Now we will study how these inverse branches behave under composition.
%     % For $ w = w_0w_1 \ldots w_n \in \{ 1,2 \}^*$ define 
%     % \begin{equation}
%     %     \label{eq:finite_word_composition_inverse_branches}
%     %     \phi_{s,w} \= \phi_{s,w_0} \circ \phi_{s,w_1} \circ \ldots \circ \phi_{s,w_n}.
%     % \end{equation} 
%     % Observe that this composition is always defined since the image of 
%     % $\phi_{s,i}$ is always contained in $D_{\theta}(J)$.
%     % Define the map
%     % $\wedge \colon \{1,2\}^* \longrightarrow \cL_{\text{Fib}} $ by 
%     % $\wedge(1) \= 12$, $\wedge(2) \= 2$ and for $w_0w_1 \ldots w_k \in 
%     % \{1,2\}^*$ we define it by concatenation, thus 
%     % $\wedge(w_0w_1 \ldots w_k) = \wedge(w_0)\wedge(w_1) \ldots 
%     % \wedge(w_k)$.  Its inverse function
%     First, we define the map
%     $\vee \colon \cL_{\text{Fib}} \longrightarrow \{ 1,2\}^*$ in the 
%     following way: If the length of $w \in \cL_{\text{Fib}}$ is one (thus 
%     $w \in \{1,2\}$), $\vee(w) = w$.
%     For $w = w_0w_1 \ldots w_n \in \cL_{\text{Fib}}$ with $n > 1$, we
%     read it from left to right, if $i < n-1$ and $w_i =1$, then $w_{i+1} =2$
%     and $\vee$ replaces $w_iw_{i+1}$ by $1$, and we continue reading 
%     $w_{i+2}$. If $w_i = 2$ then $\vee$ keeps the symbol and continue
%     reading $w_{i+1}$. The map $\vee$ stops once it moves beyond the last
%     symbol. If $\vee$ reads $w_n$, then it keeps it.

%      Fix $s \in \Omega$ and $\bf{w} = (w_i)_{i \geq 0} \in \SFib$. 
%     Since, for $i \in \{ 1,2\}$, and every $x \in D_{\theta}(J)$ we have that
%     $\phi_{s,i}(x) \in D_{\theta}(K_i)$, and 
%     $f_s(\phi_{s,1}(x)) \in D_{\theta}(K_2)$, it follows that, for every 
%     $k \geq 0$
%     \begin{equation}
%     \label{eq:finite_itineraries_using_inverse_branches}
%     \phi_{s,\vee(\bf{w}|_{[0,k]})}(D_{\theta}(J)) = \{ x \in D_{\theta}(J) \colon 
%     f_s^i(x) \in D_{\theta}(J_{w_i}) \text{ for } i = 0,1, \ldots, k \}.
%     \end{equation}
%     Moreover, since for every $k,n \in \N_0$ with $n \leq k$ we have 
%     \begin{equation}
%         \vee(\bf{w}|_{[0,n]})|_{\{i\}} = \vee(\bf{w}|_{[0,k]})|_{\{i\}},
%     \end{equation}
%     for $i = 0,1, \ldots, |\vee(\bf{w}|_{[0,n]})|-1$. Then
%     \begin{align*}
%         \phi_{s,\vee(\bf{w}|_{[0,k]})}(D_{\theta}(J)) & = 
%         \{ x \in D_{\theta}(J) \colon f_s^i(x) \in D_{\theta}(K_{w_i}) 
%         \text{ for } i = 1,2, \ldots, k-1 \} \\
%         &\subseteq \{ x \in D_{\theta}(J) \colon f_s^i(x) \in 
%         D_{\theta}(K_{w_i}) \text{ for } i = 1,2, \ldots, n-1 \} \\
%         &= \phi_{s, \vee(\bf{w}|_{[0,n]})}(D_{\theta}(J)).
%     \end{align*}
%     In particular, for all $n \in \N_0$, we have
%     \begin{equation}
%         \label{eq:nested_sequence}
%         \phi_{s,\vee(\bf{w}|_{[0,n+1]})}(D_{\theta}(J)) \subseteq 
%         \phi_{s,\vee(\bf{w}|_{[0,n]})}(D_{\theta}(J)).
%     \end{equation}
    
%     % Then, as $\phi_{s,1}$ and $\phi_{s,2}$ are strict contractions of the 
%     % hyperbolic metric on $d_{D_{\theta}(J)}$, it follows that 
%     % \begin{equation}
%     %     \label{eq:hyperbolic_diameter_limit}
%     %     \lim_{n \to \infty}\diam_{d_{D_{\theta}(J)}}(\phi_{s,\vee([\bf{w}]_n)}
%     %     (D_{\theta}(J))) = 0.
%     % \end{equation}
%     % And since the hyperbolic metric $d_{D_{\theta}(J)}$ is comparable with 
%     % the euclidean metric in $\C$, we get that
%     % \begin{equation}
%     %     \label{eq:euclidean_diameter_limit}
%     %     \lim_{n \to \infty}\diam(\phi_{s,\vee([\bf{w}]_n)}(D_{\theta}(J)))=0.
%     % \end{equation}
%     % Now, by (add a reference to preliminaries) and \eqref{eq:nested_sequence},
%     % for every $i \geq 1$ and every integers $0 \leq n < k$
%     % \begin{align*}
%     %     d(\phi_{s,\vee([\bf{w}]_k)}, \phi_{s,\vee([w]_n)}) & = 
%     %     \rho (\phi_{s,\vee([\bf{w}]_k)} - \phi_{s,\vee([\bf{w}]_n)}) \\
%     %     &\leq M_i(\phi_{s,\vee([\bf{w}]_k)}- \phi_{s,\vee([\bf{w}]_n)}) +
%     %     \frac{1}{2^i}\\
%     %     &\leq \diam(\phi_{s,\vee([\bf{w}]_n)}(D_{\theta}(J))) + \frac{1}{2^i}.
%     % \end{align*}
%     % Let $\e >0$. By \eqref{eq:euclidean_diameter_limit}, we can choose 
%     % $N_0 > 1$ such that 
%     % \[\diam(\phi_{s,\vee([\bf{w}]_n)}(D_{\theta}(J))) + \frac{1}{2^n} < \e,\]
%     % for every $n \geq N_0$. Thus, $\{ \phi_{s,\vee([\bf{w}]_n)} \}_{n \geq 0}$
%     % is a Cauchy sequence. Then, there exists 
%     % $\phi_{s,\bf{w}} \in \cH(D_{\theta}(J))$ such that 
%     % $\phi_{s,\vee([\bf{w}]_n)}$ converges to $\phi_{s,\bf{w}}$ in the metric
%     % $d$, thus it converges to $\phi_{s,\bf{w}}$ uniformly on compact subsets
%     % $D_{\theta}(J)$. Also, for all $x, y \in D_{\theta}(J)$ we have 
%     % \begin{align*}
%     %     |\phi_{s,\bf{w}}(x) - \phi_{s,\bf{w}}(y)| &= \lim_{n \to \infty}
%     %     |\phi_{s,\vee([\bf{w}]_n)}(x) - \phi_{s,\vee([\bf{w}]_n)}(y)| \\ 
%     %     &\leq \lim_{n \to \infty} \diam (\phi_{s,\vee([\bf{w}]_n)} 
%     %     (D_{\theta}(J))) \\ 
%     %     &= 0.
%     % \end{align*}
%     % This implies that for all $\bf{w} \in \SFib$, the map 
%     % $\phi_{s, \bf{W}} \in \cH(D_{\theta}(J))$ is a constant map.


%     % It follows that, for every $\bf{w} \in \SFib$, and every $n \geq 0$
%     % \[ \overline{\phi_{s,\vee([\bf{w}]_{n+1})}(D_{\theta}(J))} \subset
%     % \phi_{s,\vee([\bf{w}]_{n})}(D_{\theta}(J)).\] Since $\phi_{s,i}$ is a 
%     % contraction with respect of the hyperbolic metric on $D_{\theta}(J)$ 
%     % for $i =1,2$, we have that 
%     % \[ \lim_{n \to \infty}\diam_{D_{\theta}(J)}(\phi_{s,\vee([\bf{w}]_{n})}(D_{\theta}(J))) = 0.\] So the sequence 
%     % $\{ \phi_{s,\vee([\bf{w}]_{n})}(D_{\theta}(J)) \}_{n \geq 0}$ converges 
%     % uniformly on compact subsets of $D_{\theta}(J)$ to a constant function
%     % $\phi_{s, \bf{w}}$.  
%     % Since $ I \setminus (K_1 \cup K_2) $ is contained in the immediate basin 
%     % of attraction of $\cO_{f_{s_0}}(c)$, it follows 
%     % \[ (\Lambda (f_{s_0}) \cap I) \subset (J_1 \cup J_2),\] and as 
%     % $\cO_{f_{s_0}}(c) \cap (J_1 \cup J_2) = \emptyset$, we have that 
%     % $x \in \Lambda(f_{s_0})\cap I$ if and only if 
%     % $\cO_{f_{s_0}}(x) \subset (J_1 \cup J_2)$.    
%     % In particular, for every $n \geq 1$,
%     % \begin{equation}
%     % \label{eq:contention_of_the_repppeller_under_inverse_branches}
%     %     (\Lambda(f_{s_0}) \cap I) \subset \cup_{w \in \cL_{\text{Fib}(n)}} 
%     %     \phi_{s_0,\vee(w)} (J),
%     % \end{equation}   
%     % By Montel's Theorem, the family 
%     % \[ \cF_{s} \= \{ \phi_{s, \vee(w)} \colon w \in \cL_{Fib} \}, \] is  
%     % normal. Since $\phi_{s,1}$ and $\phi_{s,2}$ depend holomorphically on 
%     % $s$. Then each accumulation point of $\cF_s$ depends holomorphically on
%     % $s$. Moreover, if we fix $s \in \Omega$, since $\phi_{s,i}$ is a
%     % univalent contraction for $i=1,2$, and for every $\bfw \in \SFib$ we have
%     % that $\phi_{s, \vee([\bfw]_n)}(J)$
%     % the sequence $\{ \phi_{s, \vee([\bfw]_n)} \}_{n \geq 0}$ converges
%     % uniformly on compact subsets of $D_{\theta}(J)$ to a constant
%     % map $\phi_{s,\bfw}$.

%     Now we prove that the action of $f_{s_0}$ restricted to 
%     $\Lambda (f_{s_0}) \cap I$ is conjugated to the action of $\sigma$ on 
%     $\SFib$. First, observe that 
%     $I \setminus (K_1 \cup K_2)$ contains $\cO_{f_{s_0}}(c)$, it has nonempty
%     interior and is contained in the immediate basin of $\cO_{f_{s_0}}(c)$.
%     It follows that  \[ (\Lambda(f_{s_0}) \cap I) \subset K_1 \cup K_2. \]
%     Thus, $x \in \Lambda (f_{s_0}) \cap I$ if and only if 
%     $\cO_{f_{s_0}}(x) \subset K_1 \cup K_2.$ Then, for every 
%     $n \geq 1$
%     \begin{equation}
%     \label{eq:contention_of_the_repppeller_under_inverse_branches}
%         (\Lambda(f_{s_0}) \cap I) \subset \bigcup_{w \in \cL_{\text{Fib}(n)}} 
%         \phi_{s_0,\vee(w)} (J),
%     \end{equation}
%     Thus $x_{s_0}(\bf{w}) \in K_1 \cup K_2$. By 
%     \eqref{eq:contention_of_the_repppeller_under_inverse_branches}, 
%     $x_{s_0}(\bf{w}) \in \Lambda(f_{s_0}) \cap I$, and by 
%     \eqref{eq:finite_itineraries_using_inverse_branches} we have that the 
%     itinerary of $x_{s_0}(\bf{w})$ under $f_{s_0}$ is equal to 
%     $(I_{w_i})_{i \geq 0}$. So we can define the map
%     \begin{align*}
%         \psi \colon \SFib &\longrightarrow \Lambda(f_{s_0}) \cap I \\
%         \bf{w} &\mapsto x_{s_0}(\bf{w}).
%     \end{align*}
%     This map is injective since if $\bf{w}, \bf{u} \in \SFib$ with 
%     $\bf{w} \neq \bf{u}$,
%     then $w_i \neq u_i$ for some $i \geq 0$. So, 
%     $J_{w_i} \cap J_{u_i} = \emptyset$, and  
%     $f_{s_0}^i(x_{s_0}(\bf{w})) \in J_{w_i}$ and 
%     $f_{s_0}^i(x_{s_0}(\bf{u})) \in J_{u_i}$. This implies that 
%     $f_{s_0}^i(x_{s_0}(\bf{w})) \neq f_{s_0}^i(x_{s_0}(\bf{u}))$. It is 
%     onto since for any $x \in \Lambda (f_{s_0}) \cap I$ with itinerary 
%     $(I_{w_i})_{i \geq 0}$, then $(w_i)_{i \geq 0} \in \SFib$, and 
%     \begin{equation}
%         \label{eq:identyti_of_the_itinerary}
%         \cI(x_{s_0}((w_i)_{i \geq 1})) = (I_{w_i})_{i \geq 0} = \cI(x).
%     \end{equation}
%     This implies that $x_{s_0}((w_i)_{i \geq 0}) = x$. Thus, $\psi$ is a bijection.
%     %%%%%% continue from here tomorrow %%%%%
    
%     To prove the continuity of $\psi$, first observe that 
%     \eqref{eq:contention_of_the_repppeller_under_inverse_branches} implies 
%     that for $w = w_0 \ldots w_{n-1} \in \cL_{\text{Fib}}(n)$ we have 
%     \[f_{s_0}^i(\phi_{s_0,\vee(w)}(J)) \subset J_{w_i},\] for 
%     $i = 0, \ldots, n-1.$
%     If $w = w_0 \ldots w_{n-1}$ and $u = u_0, \ldots, u_{n-1}$ are in 
%     $\cL_{\text{Fib}}(n)$ with $w \neq u$, thus $w_i \neq u_i$ for some 
%     $i \in \{ 0,1, \ldots, n-1 \}$, then 
%     \[ f_{s_0}^i(\phi_{s_0,\vee(w)}(J)) \cap f_{s_0}^i(\phi_{s_0,\vee(u)}(J))
%     = \emptyset.\] This implies that 
%     $\phi_{s_0,\vee(w)}(J) \cap \phi_{s_0,\vee(u)}(J) = \emptyset$. So the 
%     number of connected components of 
%     \[ \bigcup_{w \in \cL_{\text{Fib}}(n)} \phi_{s_0,\vee(w)}(J)  \] is equal
%     to the nth Fibonacci number $\ell_n$. Put 
%     \[ d_n \= \max_{w \in \cL_{\text{Fib}(n)}} \diam_{D_{\theta}(J)}
%     (\phi_{s_0,\vee(w)}(J)).\] 
%     Since for every $\bf{w} \in \SFib$ the sequence 
%     $\{ \phi_{s,\bf{w}|_{[0,k]}} \}_{k \geq 0}$ converges uniformly on 
%     $D_{\theta}(J)$ to a constant function, it follows that
%     $d_n \rightarrow 0$ as 
%     $n \rightarrow \infty$. Let $\e > 0$. Choose $n$ large enough
%     so that $d_n < \e$. Taking $\delta = 2^{-n}$, we have that
%     any two sequences $\bf{u}, \bf{v} \in \SFib$
%     with $\dist(\bf{u},\bf{v}) < 2^{-n}$ belong to a cylinder
%     $[w]$ with $w \in \cL_{\text{Fib}}(n)$. Then 
%     \[ \dist_{D_{\theta}(J)}(\phi_{s_0,\bf{u}}, \phi_{s_0,\bf{v}}) < 
%     d_n < \e. \]
%     Thus, $\psi$ is continuous.

%     Since $\SFib$ and $\Lambda(f_{s_0}) \cap I$ are compact spaces, and
%     $\psi$ is a continuous bijection, we have that $\psi^{-1}$ is also 
%     continuous.
    

%     Finally, observe that by \eqref{eq:finite_itineraries_using_inverse_branches}, it follows that 
%     for any $\bf{w} \in \SFib$ we have 
%      $\psi(\sigma (\bf{w})) = f_{s_0}(\psi(\bf{w}))$. So $\psi$ is a
%      topological conjugacy between the action of $f_{s_0}$ on 
%      $\Lambda (f_{s_0}) \cap I$ and $\SFib$.

%     The construction above carries without changes to $f_s$ for 
%     $s \in \Omega \cap \R$. Since we chose $\Omega$ small enough 
%     so that for $s \in \Omega \cap \R$ the map $f_s$ has a periodic attracting
%     cycle of minimal period three close enough to $\cO_{f_{s_0}}(c)$ so that 
%     $\Lambda (f_s) \cap I$ is contained in $K_1 \cup K_2$ and 
%     $\Crit (f_s) \cap (K_1 \cup K_2) = \emptyset$.

    
%     Now we will construct the holomorphic motion of 
%     $\Lambda (f_{s_0}) \cap I$. Consider the map
%     \[ h \colon \Omega \times (\Lambda_{f_{s_0}} \cap I) \longrightarrow \CC, \] defined 
%     as $h(s,x) \= \phi_{s,\vee(\cI(x))}$ for every 
%     $(s,x) \in \Omega \times (\Lambda (f_{s_0}) \cap I)$.
%     We have to prove that
%     \begin{enumerate}
%         \item $h(s_0,x) = x$ for every $x \in \Lambda_{s_0}$,
%         \item $x \mapsto h(s,x)$ is injective for every $s \in \Omega$, and 
%         \item $s \mapsto h(s,x)$ is holomorphic for any $x \in \Lambda_{s_0}$.
%     \end{enumerate}
    
%     For (1), observe that by \eqref{eq:identyti_of_the_itinerary}, for every 
%     $x \in \Lambda (f_{s_0}) \cap I$, we have 
%     $h(s_0,x) = \phi_{s_0,\cI(x)} = x.$

%     To prove (2), fix $s \in \Omega$. By definition, for every 
%     $x \in \Lambda (f_{s_0}) \cap I$ we have 
%     $\cI(h(s,x)) = \cI(\phi_{s,\cI(x)}) = \cI(x)$. Since for 
%     $x, y \in \Lambda (f_{s_0}) \cap I$, with $x \neq y$, we have 
%     $\cI(x) \neq \cI(y)$, the above implies that $h(s,x) \neq h(s,y)$.

%     For (3), fix $x \in \Lambda (f_{s_0}) \cap I$. By Montel's Theorem, the
%     family \[ \cF \= \{ \phi_{s, \vee(w)} \colon w \in \cL_{\text{Fib}} \, 
%     \text{ and } s \in \Omega \} \]
%     is normal, and each $\phi_{s, \vee(w)}$ is holomorphic in $s$, we have 
%     that every limit point of $\cF$ depends holomorphically on $s$. In 
%     particular, for fixed $x \in \Lambda (f_{s_0}) \cap I$, the map
%     $\phi_{s, \cI(x)}$ is holomorphic in $s$.

%     Thus, $h$ is a holomorphic motion of $\Lambda_{s_0}$ parametrized by 
%     $\Omega$. 
%     This concludes the proof of the lemma.
    


    
   

    
%     %%%%%%%%%%%%%%%%%%%%%%%% CURRENT PROOF STATE%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % \vspace{1cm}
%     % By Schwarz-Pick Lemma, 
%     % $\phi_{s_0,i}$ is a uniform contraction in $D_{\theta}(J)$
%     % with respect to the hyperbolic metric $\dist_{D_{\theta}(J)}$, 
%     % for $i =1,2$. 

%     % For $ w = w_0w_1 \ldots w_n \in \{ 1,2 \}^*$ define 
%     % \begin{equation}
%     %     \label{eq:finite_word_composition_inverse_branches}
%     %     \phi_{s_0,w} = \phi_{s_0,w_0} \circ \phi_{s_0,w_1} \circ \ldots \circ \phi_{s_0,w_n}.
%     % \end{equation} 
%     % So, for $w \in \cL_{\text{Fib}}$ we have
%     % \[ \phi_{s_0,\vee(w)}(J) = \{ x \in J \colon 
%     % f_s^i(x) \in J_{w_i} \text{ for } i = 0,1, \ldots, n \}. \]
%     % In particular, for every $n \geq 1$,
%     % \[ \Lambda(f_{s_0}) \subseteq \cup_{w \in \cL_{\text{Fib}(n)}} 
%     % \phi_{s_0,\vee(w)} (J). \]

%     % By Schwarz-Pick Lemma, 
%     % $\phi_{s_0,i}$ is a uniform contraction for $i = 1,2$, with respect to the 
%     % hyperbolic metric on $D_{\theta}(J)$. As the Euclidean metric, and 
%     % $\dist_{D_{\theta}(J)}$ are comparable, we have that the Euclidean diameter
%     % of $\phi_{s_0,\vee([\bfw]_n)}$ goes to zero as $n$ goes to infinity. Then,
%     % for any $\bfw \in \SFib$, the limit
%     % \begin{equation}
%     % \label{eq:infinit_word_composition_inverse_branches}
%     % \phi_{s_0,bfw} \= \lim_{n \to \infty} \phi_{s_0,\vee([bfw]_n)},    
%     % \end{equation}
%     % where $[\bfw]_n$ represents the finite word of length $n+1$ that coincide
%     % with the first $n+1$ symbols of $\bfw$, is a constant function,
%     % and \[ \cI(\phi_{s_0, \bfw}) = \bfw.\] In particular, the map 
%     % $\bfw \mapsto \phi_{s_0, \bfw}$, is an homeomorphism conjugating $f_{s_0}$
%     % and $\sigma$.

%     % Now we construct a holomorphic motion of $\Lambda(f_{s_0}) \cap I$ on a 
%     % neighborhood of $s_0$.
    
%     % Fix a $\theta \in (0, \pi)$. As $f_s$ depends analytically on 
%     % $s \in [a,b]$, we can find a domain $\Omega \subset \C$ containing $s_0$
%     % such that for every $s \in \Omega$ we have 
%     % \[ D_{\theta}(J_2) \subset f(D_{\theta}(J_1)) \hspace{0.5cm} \text{ and }
%     % D_{\theta}(J) \subset f(D_{\theta}(J_2)).\] So, we can define the inverse 
%     % branch of $f_s$ and $f^2_s$ restricted to $D_{\theta}(J)$. They extend 
%     % uniquely to the slit plane $\C_{J}$ and 
%     % \[ \phi_{s,i}(D_{\theta}(J)) \subset D_{\theta}(J_i), \] for $i =1,2.$
%     % For every $s \in \Omega$ and $w \in \cL_{\text{Fib}}$, we define
%     % $\phi_{s,w}$ as in \eqref{eq:finite_word_composition_inverse_branches}. 
%     % Again, by Schwarz-Pick Lemma, we can define $\phi_{s,\bfw}$ as in 
%     % \eqref{eq:infinit_word_composition_inverse_branches} and is a constant 
%     % function for every $\bfw \in \SFib$.
     

       
%     % By Lemma \ref{lemm:Schwarz_Lemma} we have  
%     % \begin{equation}
%     %     \label{eq:Schwarz_Lemma}
%     %     \phi_i(D_{\theta}(J)) \subset D_{\theta}(J_i), 
%     % \end{equation}
%     % for $i =1,2$. 
    
    
%     % { \color{red} ADD THIS TO THE PRELIMINARIES ABOUT THE FIBONACCI SHIFT 
%     % TOGETHER WITH LEMMA 4.6
%     % Let $\cL_{\text{Fib}} $ be the set of finite words  
%     % $\bfw = w_0w_1 \ldots w_{|\bfw|} \in \{1,2\}^*$ such that 
%     % $w_iw_{i+1} \neq 11$ for every $0 \leq i < |\bfw|$, and let 
%     % $\cL_{\text{Fib}}(n)$ be the set of words in $\cL_{\text{Fib}}$ of length
%     % $n$. Define the map
%     % % $\wedge \colon \{1,2\}^* \longrightarrow \cL_{\text{Fib}} $ by 
%     % % $\wedge(1) \= 12$, $\wedge(2) \= 2$ and for $w_0w_1 \ldots w_k \in \
%     % %{1,2\}^*$ we define it by concatenation, thus 
%     % % $\wedge(w_0w_1 \ldots w_k) = \wedge(w_0)\wedge(w_1) \ldots 
%     % %\wedge(w_k)$.  Its inverse function 
%     % $\vee \colon \cL_{\text{Fib}} \longrightarrow \{ 1,2\}^*$ in the 
%     % following way: For $\bfw = w_0w_1 \ldots w_n \in \cL_{\text{Fib}}$ we
%     % read it from left to right, if $i < n-1$ and $w_i =1$, then $w_{i+1} =2$
%     % and $\vee$ replaces $w_iw_{i+1}$ by $1$, and we continue reading 
%     % $w_{i+2}$. If $w_i = 2$ then $\vee$ keeps the symbol and continue
%     % reading $w_{i+1}$. The map $\vee$ stops once it moves beyond the last
%     % symbol. If $\vee$ reads $w_n$, then it keeps it.}
    
   

%     % Now we will prove that the inverse branches are contracting and that the
%     % limits of compositions are indeed constant.
%     % The inverse branches, $\phi_1$ and $\phi_2$, of $f$ and $f^2$ 
%     % respectively, extend uniquely to $\C_{J}$. So 
%     % \[ \phi_1 \colon \C_{J} \longrightarrow \C_{J_1} \hspace{0.5cm} 
%     % \text{ and } \hspace{0.5cm} \phi_2 \colon \C_{J} 
%     % \longrightarrow \C_{J_2},\] are analytic. Fix a $\theta \in (0, \pi)$.  
%     % By Lemma \ref{lemm:Schwarz_Lemma} we have  
%     % \begin{equation}
%     %     \label{eq:Schwarz_Lemma}
%     %     \phi_i(D_{\theta}(J)) \subset D_{\theta}(J_i), 
%     % \end{equation}
%     % for $i =1,2$. 
    
%     % By Montel's Theorem, the family 
%     % \[ \cF \= \{ \phi_{\vee(\bfw)} \colon \bfw \in \cL_{\text{Fib}} \}, \]
%     % is a normal family. Now, for any $\ulw \in \SFib$, let
%     % \begin{equation}
%     % \label{eq:infinit_word_composition_inverse_branches}
%     % \phi_{\ulw} \= \lim_{n \to \infty} \phi_{\vee([\ulw]_n)},    
%     % \end{equation}
%     % where
%     % $[\ulw]_n$ represents the finite word of length $n+1$ that coincide with
%     % the first $n+1$ symbols of $\ulw$. Since $\hI$ is a geodesic of 
%     % $D_{\theta}(\hI)$, by \eqref{eq:Schwarz_Lemma}, $\phi_i$ decreases the 
%     % hyperbolic distance. As the Euclidean and hyperbolic distances are 
%     % comparable, we have that $\phi_{\vee([\ulw]_n)}$ decreases as $n$ goes to
%     % infinity. Thus, $\phi_{\ulw}$ is a constant function for every 
%     % $\ulw \in \SFib$ and \[ \cI(\phi_{\ulw}) = \ulw. \] So, the map
%     % $\tau \colon \SFib \longleftrightarrow \Lambda (f) \cap I$, given by
%     % \[ \tau (\ulw) = \phi_{\ulw}(\hI), \] is an homomorphism.

    
%     % Finally, we will prove that $\Delta (f) \cap I$ depends analytically on 
%     % $s$ on a neighborhood of $s_0$.
%     % Since the inverse branches $\phi_1$ and  $\phi_2$ of $f$ depends 
%     % continuously on the parameter, we can find a domain 
%     % $\Omega \subset \C$ containing $s_0$ such that for every $s \in \Omega$
%     % and any $\theta \in (0, \pi)$ there are 
%     % \[D(s) \subset D_{\theta}(\hI) \hspace{0.3cm} \text{ and } 
%     % \hspace{0.3cm} D_i(s) \subset D_{\theta}(\hI_i), \] with $i = 1,2$, 
%     % for which the inverse branches $\phi_{s1}$ and $\phi_{s2}$ of $f_s$
%     % restricted to $D(s)$ satisfy $\phi_{si}(D(s)) \subset D(s)$. So, for each
%     % $s \in \Omega$, we can define $\phi_{s\bfw}$, for 
%     % $\bfw \in \cL_{\text{Fib}}$, as in \eqref{eq:finite_word_composition_inverse_branches}, and 
%     % $\phi_{s\underline{\bfw}}$, for $\underline{\bfw} \in \SFib$, as in 
%     % \eqref{eq:infinit_word_composition_inverse_branches}. Then, 
%     % \[ \cF_s \= \{ \phi_{s\vee(\bfw)} \colon \bfw \in \cL_{\text{Fib}} \},\]
%     % is a normal family, and as before, for any $ \underline{\bfw} \in \SFib$
%     % we have that $\phi_{s\underline{\bfw}}$ is a constant function. In 
%     % particular, this proves that $\Lambda_{s_0}$ depends analytically on 
%     % $s \in \Omega$.
                
% \end{proof}

%%%%%%%%%%%GRAPH OF THE CONSTRUCTION OF THE INVERSE BRANCHES%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[h!]
%   \centering
%     \begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=3.3cm,y=4cm]
%     \clip(-1.7606566481216794,-.5290389905687337) rectangle (2.06076906654733,0.3050905534000426);
% \draw [line width=1pt] (-1.6283250703999999,0)-- (1.87052,0);
% \draw [line width=1pt] (-1.5,-0.2)-- (1.7,-0.2);
% \draw [line width=1pt] (-1.35,-0.4)-- (-0.15,-0.4);
% \draw [line width=1pt] (0.12,-0.4)-- (1.55,-0.4);
% \draw [line width=0.5pt, dashed] (-1.5,0)-- (-1.5,-0.2);
% \draw [line width=0.5pt, dashed] (1.7,0)-- (1.7,-0.2);
% \draw [line width=0.5pt, dashed] (-1.35,0)-- (-1.35,-0.4);
% \draw [line width=0.5pt, dashed] (-0.15,0)-- (-0.15,-0.4);
% \draw [line width=0.5pt, dashed] (0.12,0)-- (0.12,-0.4);
% \draw [line width=0.5pt, dashed] (1.55,0)-- (1.55,-0.4);
% %\draw [line width=2pt] (0,0.08193371459071828)-- (0,-0.85);

% %%%%%%%%%%%%%%%%%%%% LABELS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{scriptsize}
% \draw [fill=black] (-1.6283250703999999,0) circle (1pt);
% \draw[color=black] (-1.6505894678493178,0.06325904625025687) node {$f^2_{s_0}(c)$};

% \draw [fill=black] (-0.25,0) circle (1pt);
% \draw[color=black] (-0.25,0.06325904625025687) node {$\hat{p}_0$};

% \draw [fill=black] (1.87052,0) circle (1pt);
% \draw[color=black] (1.917382237811931,0.06325904625025687) node {$f_{s_0}(c)$};

% \draw [fill=black] (-1.05,0) circle (1pt);
% \draw[color=black] (-1.05,0.06325904625025687) node {$p_2$};

% \draw [fill=black] (-1.25,0) circle (1pt);
% \draw[color=black] (-1.25,0.06325904625025687) node {$\ell_0$};

% \draw [fill=black] (-1.35,0) circle (1pt);
% \draw [fill=black] (-1.35,-0.4) circle (1pt);
% \draw[color=black] (-1.35,-0.48) node {$\ell_1$};
% \draw[color=black] (-0.75,-0.33) node {$J_1$};

% \draw [fill=black] (-1.5,0) circle (1pt);
% \draw [fill=black] (-1.5,-0.2) circle (1pt);
% \draw[color=black] (-1.5,-0.28) node {$f^3_{s_0}(\ell_0)$};

% \draw [fill=black] (1.7,0) circle (1pt);
% \draw [fill=black] (1.7,-0.2) circle (1pt);
% \draw[color=black] (1.7,-0.28) node {$f^2_{s_0}(\ell_1)$};

% \draw [fill=black] (-0.15,0) circle (1pt);
% \draw [fill=black] (-0.15,-0.4) circle (1pt);
% \draw[color=black] (-0.18,-0.48) node {$\widehat{f_{s_0}(\ell_0)}$};

% \draw [fill=black] (0.45,0) circle (1pt);
% \draw[color=black] (0.45,0.06325904625025687) node {$p_0$};

% \draw [fill=black] (0.22,0) circle (1pt);
% \draw[color=black] (0.22,0.06325904625025687) node {$f_{s_0}(\ell_0)$};

% \draw [fill=black] (0.12,0) circle (1pt);
% \draw [fill=black] (0.12,-0.4) circle (1pt);
% \draw[color=black] (0.16,-0.48) node {$f_{s_0}(\ell_1)$};
% \draw[color=black] (0.77,-0.33) node {$J_2$};

% \draw [fill=black] (1.35,0) circle (1pt);
% \draw[color=black] (1.35,0.06325904625025687) node {$p_1$};

% \draw [fill=black] (1.55,0) circle (1pt);
% \draw [fill=black] (1.55,-0.4) circle (1pt);
% \draw[color=black] (1.55,-0.48) node {$f^2_{s_0}(\ell_0)$};

% \draw[color=black] (0,0.06325904625025687) node {$c$};
% \draw[color=black] (0,0.12325904625025687) node {$J$};
% \draw[color=black] (0,-0.13325904625025687) node {$I$};
% \draw [fill=black] (0,0) circle (1pt);
% \end{scriptsize}
% \end{tikzpicture}
%    \caption{Diagram of the intervals 
%    $I = [f_{s_0}^2(c), f_{s_0}(c)]$ on top, 
%    $J = [f_{s_0}^3(\ell_0), f_{s_0}^2(\ell_1)]$ on the second level,
%    $J_1 = [\ell_1, \widehat{f_{s_0}(\ell_o)}]$, and 
%    $J_2 = [f_{s_0}(\ell_1), f_{s_0}^2(\ell_0)]$ on the third level.}
%   \label{fig:intervals_Js}
% \end{figure}




%%%%%%%%%%%%%%%%%% OLD PROOF%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Now we will prove that there are values $s \in (1, s_*)$ for which $\cI(c_s)$
% is nonperiodic, and thus the forward orbit of $c_s$ does not converge to a 
% periodic orbit, so $F_s$ is not hyperbolic. We start recalling some
% definitions.

% Since $F_s([\beta_s,1]) = [-s,1]$, and $F_s([-s,1]) = [-s,1]$, we will 
% consider the action of $F_s$ on the interval $[-s,1]$.

% A periodic point $p$ of $F_s$ (or the cycle $\cO_{F_s} (p)$) is called 
% \emph{attracting} if its \emph{basin}, defined as the set 
% \[ \cB(p) \= \{x \in I \colon p \in \omega_{F_s}(x) \}, \] contains an open 
% set. 
% The \emph{immediate basin} of $p$ is the union of the connected 
% components of its basin intersection $\cO_{F_s}(p)$. The 
% \emph{hyperbolic set} or \emph{repeller} of $F_s$ is the set
% \[ \Lambda_s \= \{ x \in [-s,1] \colon F^n_s(x) \notin \cB(0) 
% \text{ for all } n \geq 0 \}. \] It is not hard to see that $\Lambda_s$ 
% is nonempty. We will show that the action of $F_s$ restricted to $\Lambda_s$
% is semi-conjugated to the action of the left shift on 
% \[ \SFib \= \{ \underline{w} \in \{ 1,2 \}^{\N_0} \colon w_iw_{i+1} \neq 
% 11 \text{ for all } i \geq 0 \}. \]
% \begin{rema}
%     The symbols on $\SFib$ were chosen so that the correspondence with 
%     $\Lambda_s$ is more clear.    
% \end{rema}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Unbounded_Lyapunov_exponent"
%%% End:


==> Sec_5_Dyn_real_poly.tex <==
\section{Dynamics of real polynomials} 
\label{sec:dyn_of_real_poly}

Thing we want to add in this section:
\begin{enumerate}
    \item General polynomial results described in Section \ref{section_the_bimodal_case}
    \item Definition of \emph{filled Julia set} and the result that for 
    real polynomial maps $f(\partial K_{\R}(f)) \subseteq \partial K_{\R}(f)$
\end{enumerate}


\begin{defi}
    \label{def:Thurston_map}
    A \emph{Thurston map} is an orientation preserving branched covering map 
    from a topological $2-$sphere onto itself for which every bench point has
    a finite orbit.
\end{defi}


==> Sec_6_VU_polynomials.tex <==
\section{Realization of virtually unimodal map} \label{sec:VU_polynomials}

In this section, we will prove the following proposition.

{\color{red} FORMULATE THE RESULTS IN TERMS OF THE EXPANSIVE COMBINATORICS AND 
REFER TO BLE'S PAPER FOR AN EXPLICIT CONSTRUCTION OF REAL HUBBARD TREES}

\begin{prop}
    For every $d \geq 3$ the set of post-critically finite
    virtually unimodal real polynomial map of degree $d$ with $d-1$ distinct 
    turning points in non-empty.
\end{prop}

Observe that, in Example \ref{example_VU_combinatorics}, we constructed a 
virtually unimodal combinatorics with $\ell$ distinct turning points for any
$\ell \geq  2$. So, to prove Proposition 
\ref{prop:VU_PCF_polynomial_realization}, is enough to prove that for any 
$\ell \geq 2$ the virtually unimodal combinatorics constructed in Example
\ref{example_VU_combinatorics}, is realizable by a post-critically finite 
polynomial of degree $d = \ell +1$.

To do this, we will use the results of Porier \cite{Porier2010_Hubbard_trees}
in the realization of abstract Hubbard trees by post-critically finite
polynomials.

Given a tree $H = (\cV, \cE)$, for every $v \in \cV$ put 
\[ \cE_{v} \= \{ e \in \cE \colon v \in e \}. \] Thus, $\cE_{v}$ is the set
of edges of $H$ that are incident at $v$. We say that a vertex $v \in \cV$
is a \emph{terminal vertex of $H$} if $\cE_v$ consists of a single edge. We 
denote by $E_H$ the set of terminal vertices of $H$.

An \emph{angled tree} is a finite tree $H$ together with a collection of maps
$\{ \theta_v \}_{v \in \cV \setminus E_H}$ such that for every 
$ v \in \cV \setminus E_H$ we have that 
\begin{itemize}
    \item $\theta_v \colon \cE_v \times \cE_v \longrightarrow \Q / \Z$;
    \item $\theta_v(e,e') = -\theta_v(e',e)$ for all $e,e' \in \cE_v$. Thus,
    $\theta_v$ is skew-symmetric;
    \item $\theta_v (e,e') = 0$ if and only if $e = e'$;
    \item $\theta_v(e,e'') = \theta_v (e,e') + \theta_v(e',e'')$, for 
    all $e,e',e'' \in \cE_v$.
    
\end{itemize}

Given an angled tree $H$, we can specify a \emph{vertex dynamics} as a map
$f \colon \cV \longrightarrow \cV$ satisfying that if two vertices 
$v,v' \in \cV$ belongs to the same edge in $\cE$, then $f(v) \neq f(v')$. We 
also consider a \emph{local degree} $d \colon \cV \longrightarrow \N$
defined as $d_H\= 1 + \sum_{v \in \cV}(d(v) - 1)$. A vertex $v \in \cV$ will
be called \emph{critical} if $d(v) > 1$, and noncritical otherwise. 
Observe that the set of critical vertices is nonempty if and only if the 
total degree of the tree is larger than one.

Given a vertex dynamics $f$ defined on $\cV$, we can extend it to a map
$f \colon H \longrightarrow H$ that carries each edge homeomorphically onto
the shortest path (with the least number of edges) joining the images of its 
vertices. Then, we require that for every $v \in \cV \setminus E_H$, and 
every $e,e' \in \cE_v$
\[ \theta_{f(v)} (f(e),(e')) = d(v) \theta_v(e,e'). \] Here we understand 
that $\theta_{f(v)}$ is evaluated at the edges of $f(e)$ and $f(e')$ that 
are incident at $f(v)$.

The orbit of a periodic critical vertex will be called \emph{critical cycle}.
We say that a vertex of $H$ is of \emph{Fatou type} (or that is a 
\emph{Fatou vertex}) if its orbit contains a critical cycle. Else, we say that
it is of \emph{Julia type} (or that is a \emph{Julia vertex}).

For $v,v' \in \cV$ we define the distance between them $\dist_H(v,v')$ as 
the number of edges in the shortest path joining $v$ with $v'$
We define a distance between vertices in $H$. We say that a vertex dynamics
$f$ defined on $H$ is \emph{expanding},
if for every edge $e \in \cE$ whose vertices $v, v'$ are of Julia type
there is $n \geq 1$ so that $\dist_H(f^n(v),f^n(v'))>1$.

An \emph{abstract Hubbard tree} (or a Hubbard tree) is an angled tree together
with a vertex dynamics that is expanding\footnote{In 
\cite{Porier2010_Hubbard_trees} the definition of abstract Hubbard tree 
requires the extra condition that angles between incident edges at a Julia
vertex needs to be normalized. Since we are dealing with real maps, each 
vertex has at most two incident edges, so there is no need to normalize the 
angles}.

In \cite{Porier2010_Hubbard_trees}, Porier gave a characterization of abstract
Hubbard trees that can be realized as Hubbard trees of post-critically 
finite polynomial (compare with 
\cite{Douady-Hubbard1993_Top_charac_of_rationa_maps},
\cite{Bruin-Schleicher2008_Hubbard_trees_quadratic_polynomials},
\cite{Bonifan-Milnor_Surtherland2021_Thuston_alg_real_poly}). 

\begin{theo}{\cite[Theorem 1.1]{Porier2010_Hubbard_trees}}
    \label{theo:polynomial_realization_Porier}
    An angled dynamical tree can be realized as the tree associated with a 
    post-critically finite polynomial if and only if it is expanding.
\end{theo}

So, we proceed by associating an angled dynamical tree to virtually unimodal
combinatorics. Given a virtually unimodal combinatorics 
$\ovra{\rho} \in \{0, \ldots, n\}^{n+1} $, we can associate to it an angled
tree with vertex dynamics given by $\ovra{\rho}$ in the following way:
\begin{itemize}
    \item Consider $\cV = \{ 0,1, \ldots , n\}$ and 
    $\cE = \{ \{i,i+1\} \}_{i=0}^{n-1}$. Put $H = (\cV, \cE)$;
    \item Set every map $\theta_i = 1$ for $i = 1,2, \ldots, n-1$;
    \item Define the vertex dynamics as $f(i) = \rho_i$ for every 
    $i = 0,1, \ldots, n$.
    \item Set $d(i) = 2$ if $i$ is a turning point of $\ovra{\rho}$ and 
    $d(i) = 1$ else.
\end{itemize}
We denote this angled tree and its vertex dynamics by $H_{\ovra{\rho}}$ and 
$f_{\ovra{\rho}}$ respectively.

By Proposition \ref{prop:connected_filled_julia_set}, we can consider 
framed combinatorics. 

\begin{lemm}
    \label{lem:expanding_VUC}
    For every $\ell \geq 2$, the vertex dynamics $f_{\ovra{\rho}_F}(\ell)$ 
    on the angled tree $H_{\ovra{\rho}_F(\ell)}$ is expanding.
\end{lemm}

\begin{proof}
    Let $ell \geq 2$. First, we observe that the set of Fatou vertices of 
    $H_{\ovra{\rho}_F(\ell)}$ is given by $\{ \ell, \ell +2, \ell +4 \}$. 
    Then, the set of edges whose vertices are of Julia type is given by
    \[ \{ \{ i,i+1 \} \colon 0 \leq i \leq \ell -2 \}. \] By construction,
    for every $1 \leq i \leq \ell - 2$ we have that
    \[ \ell + 2 \in \langle f_{H_{\ovra{\rho}_F(\ell)}}(i), 
    f_{H_{\ovra{\rho}_F(\ell)}}(i+1) \rangle. \] Then, 
    
    \[ \dist_{H_{\ovra{\rho}_F(\ell)}}(f_{H_{\ovra{\rho}_F(\ell)}} (i), 
    f_{H_{\ovra{\rho}_F(\ell)}}(i+1)) = 2. \] Also, since 
    $\ovra{\rho}_{H_{\ovra{\rho}_F(\ell)}}$ is framed, we have that 
    $f_{H_{\ovra{\rho}_F(\ell)}}(0) = 0$. So, 
    \[ \ell \in \langle f_{H_{\ovra{\rho}_F(\ell)}}(0), 
    f_{H_{\ovra{\rho}_F(\ell)}}(1) \rangle. \] In particular, this implies
    that  
    \[ \dist_{H_{\ovra{\rho}_F(\ell)}}(f_{H_{\ovra{\rho}_F(\ell)}} (0), 
    f_{H_{\ovra{\rho}_F(\ell)}}(1)) > 1. \]
    This proves that the vertex dynamics is expanding on 
    $H_{{\ovra{\rho}_F(\ell)}}$.

\end{proof}

\begin{proof}[ Proof of Proposition \ref{prop:VU_PCF_polynomial_realization}]
    Let $d \geq 3$. Consider the virtually unimodal combinatorics with $d-1$ 
    turning points $\ovra{\rho}_F(d-1)$, and let 
    $H_{\ovra{\rho}_F(d-1)}$, $f_{\ovra{\rho}_F(d-1)}$ its associated angled
    tree and vertex dynamics.

    By Lemma \ref{lem:expanding_VUC} and Theorem 
    \ref{theo:polynomial_realization_Porier}, there exists a post-critically
    finite polynomial map $P_{\ovra{\rho}_F(d-1)}$ whose Hubbard tree coincide
    with $H_{\ovra{\rho}_F(d-1)}$, and the restriction of 
    $P_{\ovra{\rho}_F(d-1)}$ to its Hubbard tree coincide with the vertex
    dynamics $f_{\ovra{\rho}_F(d-1)}$. 

    Since the Hubbard tree of $P_{\ovra{\rho}_F(d-1)}$ is embedded in the 
    real line $\R \subset \C$, the polynomial must have real coefficients 
    (see \cite[Example 4.9]{Porier2010_Hubbard_trees}). Moreover, 
    the combinatorics of $P_{\ovra{\rho}_F(d-1)}$ is given by $\ovra{\rho}$. 
    In particular, $P_{\ovra{\rho}_F(d-1)}$ is virtually unimodal and it has
    $d-1$ distinct critical point (marked as the turning points of 
    $\ovra{\rho}_F(d-1)$).

    Finally, by construction, each of the $d-1$ turning points has degree
    $2$. So, each turning point of $P_{\ovra{\rho}_F(d-1)}$, seeing as a 
    critical point, is simple. This implied that $P_{\ovra{\rho}_F(d-1)}$ is
    a polynomial of degree $d$.
\end{proof}

==> The_post-critical_set.tex <==
\section{The set $\overline{\cO_T(c)}$}
\label{sec:post-critical}
\subsection{The combinatorics of the set $\overline{\cO_T(c)}$}
In this section, we will give an explicit description of the set $\overline{\cO_{T(c)}}$  following \cite{LyMi93}.

Put  $S(-2) = 0$ and $S(-1) = 1$.
From (\ref{eq:cut_time}) we obtain that for every $k \geq 0$ the points $c_{S(k)}$ and $c_{S(k+2)}$ are on opposite sides of $c$. Since \[ c_{S(1)} = c_2 < c < c_1 =c_{S(0)}, \]
we conclude that for $k \equiv 0 \pmod 4,~c_{S(k)}$ is to the right of $c$ and if $k \equiv 2 \pmod4 $,~$c_{S(k)}$ is to the left of $c$. Since we also know that $c_{S(1)}$ is to
the left of $c$, we can conclude that for $k \equiv 1 \pmod 4$, $c_{S(k)}$ is to the left of $c$, and for $k \equiv 3 \pmod 4$, $c_{S(k)}$ is to the right of $c$. From this, we can
conclude that if $k$ is even the points $c_{S(k)}$ and $c_{S(k+1)}$ are in opposite sides of $c$, and therefore \[ [c_{S(k+1)}, c_{S(k)}]  \supseteq [c_{S(k+2)} , c_{S(k)}].  \] In the
case that $k$ is odd, $c_{S(k)}$ and $c_{S(k+1)}$ are on the same side with respect to $c$, and therefore \[ [c_{S(k+1)} , c_{S(k)}] \subseteq [c_{S(k+2)} , c_{S(k)}].  \]

For each $k \geq 0$ let $I_k$ be the smallest closed interval containing all of the points $c_{S(l)}$ for every $l \geq k$. For each $n \geq 0$ define $I^n_k \= T^n(I_k)$. By the
above discussion  
\begin{equation}
  \label{eq:I_K}
  I_k =
  \begin{cases}
    [c_{S(k)} , c_{S(k+1)}] \text{ if  $k$ is even, } \\
    [c_{S(k)}, c_{S(k+2)}]  \text{ if $k$ is odd. }
  \end{cases}
\end{equation}

\begin{lemm}
  \label{lemm:T_injective}
  For every $k \geq 1$, we have that $T^j$ is injective on $[c_1,c_{S(k)+1}]$. In particular $I_k^{j+1} = [c_{j+1},c_{S(k) + 1 + j}]$ for every $j \in \{1, \ldots, S(k-1)-1 \}.$ 
\end{lemm}
\begin{proof}
Since $|c - c_{S(k)}| > |c - c_{S(m)}|$  and $|T([c_{S(k)},c])| = \lambda|c - c_{S(k)}|$, for every $0 \leq k < m$ we get that $c_{S(k) +1} < c_{S(m) + 1} < c_1$, in particular
$I^1_k = [c_1, c_{S(k) +1}]$. In the case $k \geq 1$, by
(\ref{eq:cut_time}), with $k$ replaced by $k+1$, for every $j \in \{ 1, \ldots , S(k-1)-1 \}$ we have that $c_{S(k)+j}$ and $c_j$ are in the same side respect to $c$. Thus
$c \notin [c_{S(k) + j}, c_j] = T^{j-1}[c_{S(k) +1} , c_1]$, and then the map $T^j$ is injective on $[c_1, c_{S(k) +1}]$. In particular, for $1 < j \leq S(k-1)$

\begin{eqnarray}
  \label{eq:interval_image_general}
  I^{j}_k & = & T^{j-1}([c_1, c_{S(k)+1}])  \\
        & = & [c_j, c_{S(k) + j}] \nonumber 
        %& = & [c_{S(k-1)}, c_{S(k+1)}]. \nonumber
\end{eqnarray}
\end{proof}
Note that for $k \geq 1$, by Lemma \ref{lemm:T_injective}, with $j = S(k-1) -1$
\begin{equation}
  \label{eq:interval_image}
  I_k^{S(k-1)} = [c_{S(k-1)}, c_{S(k) + S(k-1)}] = [c_{S(k-1)}, c_{S(k+1)}].
\end{equation}
Then, by (\ref{eq:cut_time}), $c \in I^{S(k-1)}_k$ and $c \notin I^n_k  $ for every $0 < n < S(k-1)$.
\begin{lemm} 
  \label{lemm:orbit_order}
  For all $k  \geq 0$ we have that \[ |c_i - c| > |c_{S(k-1)} - c|,\] for all $ 0 < i < S(k)$, with $i \neq S(k-1).$ 
\end{lemm}

\begin{proof}
  We will use induction on $k$. The cases $k = 0\text{ and } 1$ are vacuously true, the cases $k = 2 \text{ and } 3$ are true by the definition of Fibonacci map and
  (\ref{def:fibonacci_2}).
  Suppose now that it is true for $k$. We will prove that is
  true for $k+1$. \newline
  \textbf{Case 1:}
  Since \[ |c_{S(k-1)} - c| > |c_{S(k)} - c|,\] we have that  \[ |c_i - c| > |c_{S(k)} - c|,  \] for all $0 < i < S(k)$.\newline
  \textbf{Case 2:} 
  Since \[ c_{S(k-1) +1} < c_{S(k) +1} < c_1 \] and $T^i$ is injective on $[c_{S(k-1) +1},c_1]$ for $0<i<S(k-2)$ by Lemma \ref{lemm:T_injective}, we have that
  $c_{S(k) +i} \in (c_{S(k-1) + i}, c_i)$, for $0 < i < S(k-2)$. By the induction hypothesis, \[ |c_i -c|>|c_{S(k-1)}-c|>|c_{S(k)} -c| \]
  and \[ |c_{S(k-1) + i} - c|>|c_{S(k-1)} - c|>|c_{S(k)} - c|, \] for $0 < i < S(k-2).$ By \ref{eq:cut_time}
  $c_i$ and $c_{S(k-1) +i}$ lie on the same side of $c$ for $0 < i < S(k-2)$.  The above implies
  that \[ |c_{S(k) + i} - c| > |c_{S(k)} - c| \] for all $0 < i < S(k-2)$.\newline
  \textbf{Case 3:}
  Since $T^{S(k-2) -1}$ is injective on $[c_{S(k-1)+1}, c_1]$ we get that $c_{S(k)+S(k-2)} \in (c_{S(k)}, c_{S(k-2)})$. Also, by (\ref{eq:cut_time}),  $c_{S(k) +S(k-2)}$ and $c_{S(k-2)}$ lie on
  the same side of $c$, and opposite to $c_{S(k)}$. Then \[ |c_{S(k) + S(k-2)} - c|<|c_{S(k-2)} - c|.\]
  Hence \[ c_{S(k-2) + 1} < c_{S(k) + S(k-2) +1} < c_1. \] So by Lemma \ref{lemm:T_injective}, $c_{S(k) + S(k-2) +i} \in (c_{S(k-2)+i} , c_i)$ for
  $0 < i < S(k-3)$. By the induction hypothesis \[ |c_i - c|>|c_{S(k)} - c| \hspace{10pt} \text{ and } \hspace{10pt} |c_{S(k-2) + i} - c|>|c_{S(k)} - c|, \] for $0<i<S(k-3).$ Since, by
  (\ref{eq:cut_time}), $c_{S(k-2) +i}$ and $c_i$ lie on the same side of $c$ for $0<i<S(k-3)$ we get \[ |c_{S(k) + S(k-2) +i} -c| > |c_{S(k)} - c|, \] for all $0<i<S(k-3).$ \newline
  \textbf{Case 4:} It remains to prove that \[ |c_{S(k) + S(k-2)} - c|>|c_{S(k)} - c|.\]
  Suppose by contradiction that \[ |c_{S(k) + S(k-2)} - c|<|c_{S(k)} - c|.\] Then $c_{S(k) +1} < c_{S(k) + S(k-2) +1} < c_ 1$. Since $T^{S(k-3) -1}$ is injective on
  $[c_{S(k) +1}, c_1]$ we get that $c_{S(k+1)} \in (c_{S(k-3)},c_{S(k) + S(k-3)})$. Noting that by (\ref{eq:cut_time}) $c_{S(k-3)}$ and $c_{S(k) + S(k-3)}$ are in the same side with respect to
  $c$ we have either \[|c_{S(k+1)}-c|>|c_{S(k) + S(k-3)}-c|>|c_{S(k)}-c| \] or \[|c_{S(k+1)}-c|>|c_{S(k-3)}-c|>|c_{S(k)}-c|, \]
  a contradiction. So we must have \[ |c_{S(k) + S(k-2)}-c|>|c_{S(k)}-c|, \] and this conclude the proof.
 \end{proof}
 Let us denote \[ J_k \= I_{k+1}^{S(k-1)} = [c_{S(k-1)}, c_{S(k+1) + S(k-1)}],\] and put \[ D_k \= [c,c_{S(k)}] \] for every $k \geq 1$. For every $n \geq 0$ we use the notation
 \begin{equation}
   \label{eq:J_k_definition}
   J^n_k \= T^n(J_k) = I^{S(k-1) + n}_{k+1}.
\end{equation}
 Note that by definition $D_{k'} \subset [c_{S(k)},c_{S(k+2)}]$, for every $k' \geq k \geq 1.$ See figure \ref{fig:2}. 
 
 \begin{figure}[h!]
  \centering
    \begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=3.3cm,y=4cm]
% \draw [color=cqcqcq,, xstep=0.2cm,ystep=0.2cm] (-1.7550529850375236,-1.6113667903735556) grid (2.098096250198763,0.5404792048718992);
\clip(-1.7606566481216794,-1.0290389905687337) rectangle (2.06076906654733,0.3050905534000426);
\draw [line width=2pt] (-1.6283250703999999,0)-- (1.87052,0);
\draw [line width=2pt] (-1.6283250703999999,-0.2)-- (0.2812059514774783,-0.2);
\draw [line width=1.5pt,dash pattern=on 1pt off 2pt] (0,-0.1)-- (1.87052,-0.1);
\draw [line width=1.5pt,dash pattern=on 1pt off 2pt] (-1.6283250703999999,-0.3)-- (0,-0.3);
\draw [line width=2pt] (-0.7809225348931643,-0.4)-- (0.2812059514774783,-0.4);
\draw [line width=1.5pt,dash pattern=on 1pt off 2pt] (-0.7809225348931643,-0.5)-- (0,-0.5);
\draw [line width=2pt] (-0.1,-0.6)-- (0.2812059514774783,-0.6);
\draw [line width=2pt] (-0.1,-0.8)-- (0.1582716909839456,-0.8);
\draw [line width=1.5pt,dash pattern=on 1pt off 2pt] (0,-0.7)-- (0.2812059514774783,-0.7);
\draw [line width=2pt] (0,0.08193371459071828)-- (0,-0.95);
\draw [line width=1.5pt,dash pattern=on 1pt off 2pt] (-0.1,-0.9)-- (0,-0.9);
\begin{scriptsize}
\draw [fill=black] (1.87052,0) circle (1pt);
\draw[color=black] (1.9165342443499325,0.06135724499302839) node {$c_{1}$};
\draw [fill=black] (-1.6283250703999999,0) circle (1pt);
\draw[color=black] (-1.6502154979238352,0.06135724499302839) node {$c_{2}$};
\draw [fill=black] (1.87052,-0.1) circle (1pt);
\draw[color=black] (1.9165342443499325,-0.04414827666653128) node {$c_{1}$};
\draw [fill=black] (-1.6283250703999999,-0.2) circle (1pt);
\draw[color=black] (-1.6502154979238352,-0.13701605769366196) node {$c_{2}$};
\draw [fill=black] (0,-0.1) circle (1pt);
\draw[color=black] (0.0471180359804952,-0.03614827666653128) node {};
\draw [fill=black] (0.2812059514774783,-0.2) circle (1pt);
\draw[color=black] (0.32954782285645334,-0.16701605769366196) node {$c_{5}$};
\draw [fill=black] (-1.6283250703999999,-0.3) circle (1pt);
\draw[color=black] (-1.6502154979238352,-0.25788383872079263) node {$c_{2}$};
\draw [fill=black] (-0.7809225348931643,-0.4) circle (1pt);
\draw[color=black] (-0.8029261372959607,-0.35875161974792334) node {$c_{3}$};
\draw [fill=black] (0.2812059514774783,-0.4) circle (1pt);
\draw[color=black] (0.32954782285645334,-0.33875161974792334) node {$c_{5}$};
\draw [fill=black] (0,-0.3) circle (1pt);
\draw[color=black] (0.0471180359804952,-0.23788383872079263) node {};
\draw[color=black] (0.1345367795373394,0.082612461093534123) node {$I_0$};
\draw[color=black] (-0.6623186905769711,-0.13434802314779552) node {$I_1$};
\draw[color=black] (0.9482035464895046,-0.16348024212066482) node {$D_0$};
\draw[color=black] (-1.0335335840149502,-0.35185354480735517) node {$D_1$};
\draw[color=black] (0.1386740102630339,-0.35272132583448584) node {$I_2$};
\draw [fill=black] (-0.7809225348931643,-0.5) circle (1pt);
\draw[color=black] (-0.8029261372959607,-0.45625714140748295) node {$c_{3}$};
\draw [fill=black] (0,-0.5) circle (1pt);
\draw[color=black] (0.05552368439942253,-0.43625714140748295) node {};
\draw [fill=black] (-0.1,-0.6) circle (1pt);
\draw[color=black] (-0.115344096627705395,-0.5671249224346136) node {$c_{13}$};
\draw [fill=black] (0.2812059514774783,-0.6) circle (1pt);
\draw[color=black] (0.32954782285645334,-0.5371249224346136) node {$c_{5}$};
\draw[color=black] (-0.379888903701013,-0.5435891068616165) node {$D_2$};
\draw[color=black] (0.10091418586163009,-0.5544568878887472) node {$I_3$};
\draw [fill=black] (-0.1,-0.8) circle (1pt);
\draw[color=black] (-0.115344096627705395,-0.7688604844888751) node {$c_{13}$};
\draw [fill=black] (0.1582716909839456,-0.8) circle (1pt);
\draw[color=black] (0.20514422625632892,-0.7688604844888751) node {$c_{8}$};
\draw [fill=black] (0,-0.7) circle (1pt);
\draw[color=black] (0.05552368439942253,-0.6379927034617443) node {};
\draw [fill=black] (0.2812059514774783,-0.7) circle (1pt);
\draw[color=black] (0.32954782285645334,-0.6679927034617443) node {$c_{5}$};
\draw[color=black] (0.06039351724535334,-0.7528301905754376) node {$I_4$};
\draw[color=black] (0.15134807637519404,-0.6619624095483069) node {$D_3$};
\draw[color=black] (-0.03357618884120714,-0.3824609915263466) node {};
\draw [fill=black] (0,0.08193371459071828) circle (1pt);
\draw[color=black] (-0.026944479775069613,0.1353269510795909) node {$c$};
\draw [fill=black] (-0.1,-0.9) circle (1pt);
\draw[color=black] (-0.115344096627705395,-0.8663660061484347) node {$c_{13}$};
\draw[color=black] (-0.08693844820877806,-0.9536979716025683) node {$D_5$};
\end{scriptsize}
\end{tikzpicture}

 \caption{First five $I_k$ (solid line), and $D_k$ (dashed line) intervals.}
  \label{fig:2}
\end{figure}
 
 \begin{lemm}
  \label{lemm:J_k}
  For all $0< k <k'$ we have $J_{k'} \subset D_{k'-1} \subset I_{k}$ and $J_{k} \cap J_{k'} = \emptyset$.
\end{lemm}
\begin{proof}
  First we will prove that $J_{k+1}$ is contained in $D_k$ and $c \notin J_{k+1}$ for every $k \geq 0$. Fix $k \geq 0$.
  By (\ref{eq:cut_time}) with $k$ replaced by $k+3$ we have $c_{S(k)}$ and $c_{S(k+2) + S(k)}$ are in the same side of $c$. Since \[ |c_{S(k+2)} - c| < |c_{S(k+1)} -c|,\] we have
  \[c_{S(k+1) +1}<c_{S(k+2) +1}<c_1.\] By Lemma \ref{lemm:T_injective}, $T^{S(k) -1}$ is injective on $I_{k+1}^1$. Then, $c_{S(k+2) + S(k)} \in (c_{S(k+2)} , c_{S(k)})$. By (\ref{eq:cut_time})
  with $k$ replaced by $k+3$, we thus conclude $c_{S(k+2) + S(k)} \in (c_{S(k)} , c)$. Then
  \[J_{k+1} = [c_{S(k)}, c_{S(k) + S(k+2)}] \subset [c, c_{S(k)}] = D_k\subset [c_{S(k)},c_{S(k+2)}] \subseteq I_k \] and $c \notin J_{k+1}$. Since, by definition, for every $k' > k$ we have
  $D_{k'-1} \subset I_{k'-1} \subset I_k$, we get \[ J_{k'} \subset D_{k'-1} \subset I_k.  \]
  Now we will prove that $J_{k+1}$ and $I_{k+1}$ are disjoint.
  If $k$ is even then $I_{k+1} = [c_{S(k+1)} , c_{S(k+3)}]$. Since $c_{S(k)}$ and $c_{S(k+1)}$ lie on opposite sides respect to $c$, we have that $c_{S(k)}$, $c_{S(k) + S(k+2)}$, and
  $c_{S(k+3)}$ lie on the same side of $c$. By (\ref{lemm:orbit_order}), with $k$ replaced by $k+4$, we get \[ |c_{S(k)} - c|>|c_{S(k) + S_{k+2}} - c|>|c_{S(k+3)} - c|. \] So
  $J_{k+1} \cap I_{k+1} = \emptyset.$ Now, if $k$ is odd $I_{k+1} = [c_{S(k+1)}, c_{S(k+2)}]$ and $c_{S(k)}$, $c_{s(k+1)}$ and $c_{S(k) + S(k+2)}$ lie on the same side of $c$. Suppose that
  $|c_{S(k+1)} - c| > |c_{S(k) + S(k+2)} - c|$, then \[[c_{S(k+1)},c_{S(k) + S(k+2)}] \subset [c_{S(k)},c_{S(k) + S(k+2)}].\] Since $T^{S(k-1)}$ is injective on $[c_{S(k)},c_{S(k) + S(k+2)}]$, then
  $T^{S(k-1)}$ is injective on \newline $[c_{S(k+1)},c_{S(k) + S(k+2)}]$. So we get \[T^{S(k-1)}([c_{S(k+1)},c_{S(k) + S(k+2)}]) = [c_{S(k+1)+S(k-1)},c_{S(k+3)}].\] Since
  $S(k+1) + S(k-1) < S(k+4),$ by
  Lemma \ref{lemm:orbit_order}, with $k$ replaced by $k+4$, we get \[|c_{S(k+1) + S(k-1)} - c|>|c_{S(k+3)} - c|.\] On the other hand, $T^{S(k-1)}(J_{k+1}) = [c_{S(k+1)}, c_{S(k+3)}]$, then
  \[T^{S(k-1)}(c_{S(k+1)}) = c_{S(k+1) + S(k-1)} \in (c_{S(k+1)} , c_{S(k+3)})\] and by (\ref{eq:cut_time}), with $k$ replaced by $k+1$, we have that $c_{S(k+1) + S(k-1)}$ and $c_{S(k-1)}$ are in
  the same side of $c$. Since $k-1 \equiv k+3  \pmod4$, we have that $c_{S(k-1)}$ and $c_{S(k+3)}$ are on the same side of $c$, so
  $c_{S(k+1) + S(k-1)} \in (c,c_{S(k+3)})$. Thus \[ |c_{S(k+1) + S(k-1)} - c|<|c_{S(k+3)} - c|, \] a contradiction. So we must have $c_{S(k) + S(k+2)} \in (c_{S(k)}, c_{S(k+1)})$ and
  \begin{equation}
    \label{eq:empty_intersection}
    J_{k+1}~\cap~I_{k+1}~=~\emptyset. 
  \end{equation}
  This conclude the proof of the lemma.
\end{proof}

Taking $k' = k+1$ in Lemma \ref{lemm:J_k} we get $J_{k+1} \subset I_k$, and then %%%by (\ref{eq:empty_intersection}) and (\ref{eq:interval_image}) we get that%%%
\begin{equation}
  \label{eq:J_k_I_k_1}
  J_{k+1} \cup I_{k+1} \subset I_k \subseteq I_k^{S(k-1)},
\end{equation}
for every $k \geq 1$
\begin{defi}
  For $k \geq 0$ let $M_k$ be the $S(k)-$fold union \[ M_k = \bigcup_{0 \leq n < S(k-1) } I^n_k \cup \bigcup_{0 \leq n < S(k-2)} J^n_k.  \]
\end{defi}

\noindent Some examples of $M_k$,
\begin{eqnarray}
  M_0 & = & I_0 \nonumber \\
      & = & [c_1, c_2], \nonumber \\
  M_1 & = & I_1 \cup J_1 \nonumber \\
      & = & [c_2, c_5] \cup [c_4,c_1], \nonumber \\
  M_2 & = & I_2 \cup I^1_2 \cup J_2 \nonumber \\
      & = & [c_3, c_5] \cup [c_4, c_1] \cup [c_2,c_7] \nonumber \\
  M_3 & = & I_3 \cup I^1_3 \cup I^2_3 \cup J_3 \cup J^1_3 \nonumber \\
      & = & [c_{13}, c_5] \cup [c_6, c_1] \cup [c_2, c_7] \cup [c_3, c_{11}] \cup [c_4, c_{12}] \nonumber \\
  M_4 & = & I_4 \cup I^1_4 \cup I^2_4 \cup I^3_4 \cup I^4_4 \cup J_4 \cup J^1_4 \cup J^2_4 \nonumber \\
      &= & [c_{13}, c_8] \cup [c_9, c_1] \cup [c_2, c_{10}] \cup [c_3, c_{11}] \cup [c_4, c_{12}] \cup [c_{14}, c_5] \cup [c_6, c_{19}] \cup [c_{20}, c_7], \nonumber 
\end{eqnarray}
\noindent and so on. 

\begin{figure}[h!]
  \centering
    \begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=3.3cm,y=4cm]
    \clip(-1.7606566481216794,-1.0290389905687337) rectangle (2.06076906654733,0.3050905534000426);
\draw [line width=2pt] (-1.6283250703999999,0)-- (1.87052,0);
\draw [line width=2pt] (-1.6283250703999999,-0.2)-- (0.34,-0.2);
\draw [line width=2pt] (1.15,-0.2)-- (1.87052,-0.2);
\draw [line width=2pt] (-1.6283250703999999,-0.4)-- (-1.26,-0.4);
\draw [line width=2pt] (-0.7809225348931643,-0.4)-- (0.34,-0.4);
\draw [line width=2pt] (1.15,-0.4)-- (1.87052,-0.4);
\draw [line width=2pt] (-1.6283250703999999,-0.6)-- (-1.26,-0.6);
\draw [line width=2pt] (-0.7809225348931643,-0.6)-- (-0.58,-0.6);
\draw [line width=2pt] (-0.1,-0.6)-- (0.34,-0.6);
\draw [line width=2pt] (1.15,-0.6)-- (1.44,-0.6);
\draw [line width=2pt] (1.6,-0.6)-- (1.87052,-0.6);
\draw [line width=2pt] (-1.6283250703999999,-0.8)-- (-1.5462762185432146,-0.8006740305557355);
\draw [line width=2pt] (-1.4,-0.8)-- (-1.26,-0.8);
\draw [line width=2pt] (-0.7809225348931643,-0.8)-- (-0.58,-0.8);
\draw [line width=2pt] (-0.1,-0.8)-- (0.1182716909839456,-0.8);
\draw [line width=2pt] (0.19,-0.8)-- (0.34,-0.8);
\draw [line width=2pt] (1.15,-0.8)-- (1.44,-0.8);
\draw [line width=2pt] (1.6,-0.8)-- (1.68,-0.8);
\draw [line width=2pt] (1.8,-0.8)-- (1.87052,-0.8);
\draw [line width=2pt] (0,0.08193371459071828)-- (0,-0.85);
\begin{scriptsize}
\draw [fill=black] (1.87052,0) circle (1pt);
\draw[color=black] (1.917382237811931,0.06325904625025687) node {$c_{1}$};
\draw [fill=black] (-1.6283250703999999,0) circle (1pt);
\draw[color=black] (-1.6505894678493178,0.06325904625025687) node {$c_{2}$};
\draw [fill=black] (1.87052,-0.2) circle (1pt);
\draw[color=black] (1.917382237811931,-0.1368155984968159) node {$c_{1}$};
\draw [fill=black] (-1.6283250703999999,-0.2) circle (1pt);
\draw[color=black] (-1.6505894678493178,-0.1368155984968159) node {$c_{2}$};
\draw [fill=black] (1.15,-0.2) circle (1pt);
\draw[color=black] (1.127113516722484,-0.1368155984968159) node {$c_{4}$};
\draw [fill=black] (0.34,-0.2) circle (1pt);
\draw[color=black] (0.38681120549685644,-0.1368155984968159) node {$c_{5}$};
\draw [fill=black] (1.87052,-0.4) circle (1pt);
\draw[color=black] (1.917382237811931,-0.33689024324388867) node {$c_{1}$};
\draw [fill=black] (-1.6283250703999999,-0.4) circle (1pt);
\draw[color=black] (-1.6505894678493178,-0.33689024324388867) node {$c_{2}$};
\draw [fill=black] (-0.7809225348931643,-0.4) circle (1pt);
\draw[color=black] (-0.8036068050867275,-0.33689024324388867) node {$c_{3}$};
\draw [fill=black] (1.15,-0.4) circle (1pt);
\draw[color=black] (1.127113516722484,-0.33689024324388867) node {$c_{4}$};
\draw [fill=black] (0.34,-0.4) circle (1pt);
\draw[color=black] (0.38681120549685644,-0.33689024324388867) node {$c_{5}$};
\draw [fill=black] (-1.26,-0.4) circle (1pt);
\draw[color=black] (-1.2137859524796921,-0.33689024324388867) node {$c_{7}$};
\draw[color=black] (0.13338332215056958,0.0513436234236121024) node {$I_0$};
\draw[color=black] (-0.6618998026278329,-0.14059826405963703) node {$I_1$};
\draw[color=black] (1.5773910588998377,-0.14059826405963703) node {$J_1$};
\draw[color=black] (-1.4732370712972787,-0.3455645576149869) node {$J_2$};
\draw[color=black] (-0.24000442291972096,-0.3455645576149869) node {$I_2$};
\draw[color=black] (1.5773910588998377,-0.3405645576149869) node {$I_2^1$};
% \draw[color=black] (-0.6335694827131932,-0.2135108789831938) node {$g$};
% \draw[color=black] (1.520567525730245,-0.2135108789831938) node {$h$};
% \draw[color=black] (-1.4338680617014676,-0.4135855237302666) node {$i$};
% \draw[color=black] (-0.2100781513318981,-0.4135855237302666) node {$j$};
% \draw[color=black] (1.520567525730245,-0.4135855237302666) node {$k$};
\draw [fill=black] (-1.6283250703999999,-0.6) circle (1pt);
\draw[color=black] (-1.6505894678493178,-0.5369648879909615) node {$c_{2}$};
\draw [fill=black] (-1.26,-0.6) circle (1pt);
\draw[color=black] (-1.2137859524796921,-0.5369648879909615) node {$c_{7}$};
\draw [fill=black] (-0.7809225348931643,-0.6) circle (1pt);
\draw[color=black] (-0.8036068050867275,-0.5369648879909615) node {$c_{3}$};
\draw [fill=black] (-0.58,-0.6) circle (1pt);
\draw[color=black] (-0.525195716808531,-0.5369648879909615) node {$c_{11}$};
\draw [fill=black] (-0.1,-0.6) circle (1pt);
\draw[color=black] (-0.125016569415566546,-0.5369648879909615) node {$c_{13}$};
\draw [fill=black] (0.34,-0.6) circle (1pt);
\draw[color=black] (0.38681120549685644,-0.5369648879909615) node {$c_{5}$};
\draw [fill=black] (1.15,-0.6) circle (1pt);
\draw[color=black] (1.127113516722484,-0.5369648879909615) node {$c_{4}$};
\draw [fill=black] (1.44,-0.6) circle (1pt);
\draw[color=black] (1.4555581951368613,-0.5369648879909615) node {$c_{12}$};
\draw [fill=black] (1.6,-0.6) circle (1pt);
\draw[color=black] (1.5872814674033882,-0.5369648879909615) node {$c_{6}$};
\draw [fill=black] (1.87052,-0.6) circle (1pt);
\draw[color=black] (1.917382237811931,-0.5369648879909615) node {$c_{1}$};
\draw[color=black] (-1.4732370712972787,-0.5337762002450147) node {$I_3^2$};
\draw[color=black] (-0.6805800387479996,-0.5337762002450147) node {$J_3$};
\draw[color=black] (0.10075722992144626,-0.5337762002450147) node {$I_3$};
\draw[color=black] (1.293198019971104,-0.5337762002450147) node {$J_3^1$};
\draw[color=black] (1.7286027015298602,-0.5337762002450147) node {$I_3^1$};
% \draw[color=black] (-1.4338680617014676,-0.6136601684773394) node {$l$};
% \draw[color=black] (-0.6702498342501558,-0.6136601684773394) node {$m$};
% \draw[color=black] (0.13004874473811845,-0.6136601684773394) node {$n$};
% \draw[color=black] (1.3071545713333719,-0.6136601684773394) node {$p$};
% \draw[color=black] (1.7473187897769227,-0.6136601684773394) node {$q$};
\draw [fill=black] (-1.6283250703999999,-0.8) circle (1pt);
\draw[color=black] (-1.6505894678493178,-0.7370395327380342) node {$c_{2}$};
\draw [fill=black] (-1.5462762185432146,-0.8006740305557355) circle (1pt);
\draw[color=black] (-1.5222231664193626,-0.7403741101504855) node {$c_{10}$};
\draw [fill=black] (-1.26,-0.8) circle (1pt);
\draw[color=black] (-1.2054495089485642,-0.7370395327380342) node {$c_{7}$};
\draw [fill=black] (-1.4,-0.8) circle (1pt);
\draw[color=black] (-1.3954980280341588,-0.7370395327380342) node {$c_{20}$};
\draw [fill=black] (-0.7809225348931643,-0.8) circle (1pt);
\draw[color=black] (-0.8136105373240809,-0.7370395327380342) node {$c_{3}$};
\draw [fill=black] (-0.58,-0.8) circle (1pt);
\draw[color=black] (-0.525195716808531,-0.7370395327380342) node {$c_{11}$};
\draw [fill=black] (-0.1,-0.8) circle (1pt);
\draw[color=black] (-0.115016569415566546,-0.7370395327380342) node {$c_{13}$};
\draw [fill=black] (0.1182716909839456,-0.8) circle (1pt);
\draw[color=black] (0.09337958991321615,-0.7370395327380342) node {$c_{8}$};
\draw [fill=black] (0.19,-0.8) circle (1pt);
\draw[color=black] (0.19509166546768288,-0.7370395327380342) node {$c_{18}$};
\draw [fill=black] (0.34,-0.8) circle (1pt);
\draw[color=black] (0.38681120549685644,-0.7370395327380342) node {$c_{5}$};
\draw [fill=black] (1.15,-0.8) circle (1pt);
\draw[color=black] (1.127113516722484,-0.7370395327380342) node {$c_{4}$};
\draw [fill=black] (1.44,-0.8) circle (1pt);
\draw[color=black] (1.455581951368613,-0.7370395327380342) node {$c_{12}$};
\draw [fill=black] (1.6,-0.8) circle (1pt);
\draw[color=black] (1.5772814674033882,-0.7370395327380342) node {$c_{6}$};
\draw [fill=black] (1.68,-0.8) circle (1pt);
\draw[color=black] (1.6956477688333436,-0.7370395327380342) node {$c_{19}$};
\draw [fill=black] (1.8,-0.8) circle (1pt);
\draw[color=black] (1.807356112150457,-0.7370395327380342) node {$c_{9}$};
\draw [fill=black] (1.87052,-0.8) circle (1pt);
\draw[color=black] (1.917382237811931,-0.7370395327380342) node {$c_{1}$};
\draw[color=black] (-1.5772548904368666,-0.8737348132244122) node {$I_4^2$};
\draw[color=black] (-1.3171578522656775,-0.8737348132244122) node {$J_4^2$};
\draw[color=black] (-0.6702498342501558,-0.8737348132244122) node {$I_4^3$};
\draw[color=black] (-0.05,-0.8737348132244122) node {$I_4$};
\draw[color=black] (0.27677015088596874,-0.8737348132244122) node {$J_4$};
\draw[color=black] (1.3071545713333719,-0.8737348132244122) node {$I_4^4$};
\draw[color=black] (1.6506160448158396,-0.8737348132244122) node {$J_4^1$};
\draw[color=black] (1.847356112150457,-0.8737348132244122) node {$I_4^1$};
\draw[color=black] (-0.03334554847198755,-0.3335556658314375) node {};
\draw [fill=black] (0,0.08193371459071828) circle (1pt);
\draw[color=black] (0.026676844952133016,0.13328517191173234) node {$c$};
\end{scriptsize}
\end{tikzpicture}
   \caption{First five levels of $M_k$.}
  \label{fig:3}
\end{figure}

From the definition, for every $k \geq 0$ the $S(k)$ closed intervals \[ I_k, I^1_k, \ldots , I^{S(k-1) -1}_k, J_k, J^1_k, \ldots , J^{S(k-2)-1}_k,\] are pairwise disjoint, each $M_k$
contains the set $\overline{\cO_T(c)}$ and they
form a nested sequence of closed sets $M_1 \supset M_2 \supset M_3 \supset \ldots$ with intersection equal to the Cantor set $\overline{\cO_T(c)}$, for a proof of these
statements see \cite[Lemma 3.5]{LyMi93}.
Now by (\ref{eq:J_k_I_k_1}) we have that for every $1 \leq m < S(k-1)$, \[ I_{k+1}^m \cup J_{k+1}^m \subset I_k^m. \] Also by (\ref{eq:J_k_definition}) for every $0 \leq n < S(k-2)$,
\[ I_{k+1}^{S(k-1) + n} = J_k^n. \] Since the sets in $M_k$ are disjoint we get that
\begin{equation}
  \label{eq:J_k_I_k}
  \cup_{A \in M_{k+1}} (A \cap I_k) = I_{k+1} \cup J_{k+1.} 
\end{equation}

% The action of $T$ restricted to $\overline{\cO_T(c)}$ is semiconjugated to the \emph{Fibonacci shift}, this is the space $\Sigma_F \= \{ \ulx \in \{ 0, 1 \}^{\N_0}
% \colon x_{i-1}x_{i} \neq 11 \text{ for every } i \in \N \}$ together with the topology generated by the cylinders \[ [a_0a_1 \ldots a_{n-1}]_k \= \{ \ulx \in \Sigma_F \colon
%   x_{k + i} = a_i \text{ for every } 0 \leq i \leq n-1\}. \] Given $x \in \overline{\cO_T(c)}$, let $M_k(x)$ be the interval of the set $M_k$
% containing $x$, then define $a_k = 0$ if $M_k(x) = I^n_k$ and $a_k = 1$ if $M_k(x) = J^n_k$ for appropiate $n$. The sequence $\ula = a_0a_1a_2 \ldots \in \Sigma_F$ is the one that
% correspond to $x \in \overline{\cO_T(c)}$. We will denote by $M_{k}^{[a_0a_1 \ldots a_n]}$ the interval of $M_k$ corresponding to the cylinder $[a_0a_1 \ldots a_n]_0 \subset \Sigma_F$. 

\subsection{Diameter estimates}
In this section we will give an estimate on how the distances $|c_{S(k)} - c|$ decrease as $k \to \infty.$
 
\begin{lemm}
  \label{lemm:diam_estimate}
  The following limit \[ \lim_{k \to \infty} \lambda^{S(k+1)}|D_k|\] exists and is strictly positive. 
\end{lemm}

\begin{proof}
  Since \[T(D_k) = T([c,c_{S(k)}]) = I_k^1,\] by (\ref{eq:interval_image}) we have that \[T^{S(k-1)}(D_k) = [c_{S(k-1)}, c_{S(k+1)}] .\]
  By (\ref{eq:cut_time}), $c_{S(k-1)}$ and $c_{S(k+1)}$ are in opposite sides of $c$. Then $D_{k-1} \cap D_{k+1} = \{c\}$, so \[T^{S(k-1)}(D_k) = D_{k-1} \cup D_{k+1} .\] Since, by
  Lemma~\ref{lemm:T_injective}, $T^{S(k-1)}$ is injective on $I_k$ and $D_k \subset I_k$ we get that \[ |T^{S(k-1)}(D_k)| = \lambda^{S(k-1)} |D_k| = |D_{k-1}| +|D_{k+1}|.\]
  For $k \geq 0$ put  $\nu_k\= |D_k| / |D_{k+1}|$. By the above we get \[ \lambda^{S(k-1)} = \nu_{k-1} + \frac{1}{\nu_k}. \] By (\ref{def:fibonacci}),
  $\nu_k > 1$, so $0 < \nu_k^{-1} <1$. Since
  $\lambda >1$, we have $\lambda^{S(k-1)} \longrightarrow \infty$ as $k \longrightarrow \infty$. Then $\nu_k \longrightarrow \infty$ as $k \longrightarrow \infty$. So
  $\lambda^{S(k-1)} - \nu_{k-1} \longrightarrow 0$ as $k \longrightarrow \infty.$ Then, if we define $C_k \=\nu_k\lambda^{-S(k)}$, we have $0 < C_k < 1$ and $C_k \nearrow 1$
  exponentially fast as $n \longrightarrow\infty.$ By definition of $\nu_k$, we have that
  \[ \frac{|D_0|}{|D_{k+1}|} = \prod_{i=0}^k \nu_i 
                            = \prod_{i=0}^k \lambda^{S(i)}C_i 
                            =\lambda^{S(k+2) - S(1)}\prod_{i=0}^kC_i. \]
  % \begin{eqnarray}
  %   \frac{|D_0|}{|D_{k+1}|} &=& \prod_{i=0}^k \nu_i \nonumber \\
  %                           &=& \prod_{i=0}^k \lambda^{S(i)}C_i \nonumber \\
  %                           &=&\lambda^{S(k+2)}\prod_{i=0}^kC_i, \nonumber
  %   \end{eqnarray}
  Then 
  \begin{equation}
    \label{eq:diameter_estimate}
    |D_{k+1}|\lambda^{S(k+2) - S(1)} = |D_0| \left[ \prod_{i = 0}^k C_i \right]^{-1}. 
  \end{equation}
  Since $ \prod_{i = 0}^k C_i $ converge to a strictly positive number as $k \longrightarrow \infty$, the proof is complete.
\end{proof}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Unbounded_Lyapunov_exponent"
%%% End:

